Correct-by-Construction Design of Contextual Robotic Missions Using Contracts

Effectively specifying and implementing robotic missions poses a set of challenges to software engineering for robotic systems. These challenges stem from the need to formalize and execute a robot's high-level tasks while considering various application scenarios and conditions, also known as contexts, in real-world operational environments. Writing correct mission specifications that explicitly account for multiple contexts can be tedious and error-prone. Furthermore, as the number of contexts, and consequently the complexity of the specification, increases, generating a correct-by-construction implementation (e.g., by using synthesis methods) can become intractable. A viable approach to address these issues is to decompose the mission specification into smaller, manageable sub-missions, with each sub-mission tailored to a specific context. Nevertheless, this compositional approach introduces its own set of challenges in ensuring the overall mission's correctness. In this paper, we propose a novel compositional framework for specifying and implementing contextual robotic missions using assume-guarantee contracts. The mission specification is structured in a hierarchical and modular fashion, allowing for each sub-mission to be synthesized as an independent robot controller. We address the problem of dynamically switching between sub-mission controllers while ensuring correctness under predefined conditions.

==> Tex/background_orig.tex <==

\section{Background}
\label{sec:background}

We provide background notions on the basic building blocks of \NAME, namely, contracts, linear temporal logic, and reactive synthesis.

\subsection{Assume-Guarantee Contracts}
\label{sec:backgroundcontracts}

Contract-based design has emerged as a design paradigm that provides formal support for building complex systems in a modular way. This support facilitates compositional reasoning, step-wise refinement of system requirements, and reuse of pre-designed components~\cite{Nuzzo15b, benveniste2018contracts, passerone2019coherent}. 

An \emph{assume-guarantee contract} (or simply \emph{contract}) $\mathcal{C}$ is a triple $(V, A, G)$, where $V$ is a set of variables, including inputs and outputs (or \emph{ports}), and $A$ (assumptions) and $G$ (guarantees) are sets of behaviors over $V$. For simplicity, we often omit $V$ and refer to contracts by their assumptions and guarantees. Assumptions $A$ describe the expected behavior from the environment, while guarantees $G$ specify the system's promised behavior under those assumptions. We represent behaviors as traces over an alphabet; assumptions and guarantees are sets of traces that satisfy logical formulas. To avoid confusion, we also use logical formulas to represent the assumptions and guarantees.

\subsubsection{Contract Refinement} 

Refinement establishes a pre-order between contracts, which formalizes the notion of replacement. Let
$\mathcal{C} = (A, G)$ and $\mathcal{C}' = (A', G')$ be two contracts; we say that $\mathcal{C}$ refines $\mathcal{C}'$, denoted by  $\mathcal{C} \preceq \mathcal{C}'$, if and only if all the assumptions of $\mathcal{C}'$ are contained in the assumptions of $\mathcal{C}$ and all the guarantees of $\mathcal{C}$ are included in the guarantees of $\mathcal{C}'$, that is, if and only if $A \supseteq A' \text{ and } G \subseteq G'$.
Refinement entails relaxing the assumptions and strengthening the guarantees. When $\mathcal{C} \preceq \mathcal{C}'$, we also say that $\mathcal{C}'$ is an \textit{abstraction} of $\mathcal{C}$ and can be replaced by $\mathcal{C}$ in the design.

\subsubsection{Contract Composition}

Contracts specifying different implementations can be combined via the composition operation ($\parallel$). Let $\mathcal{C}_1 = (A_1, G_1)$ and $\mathcal{C}_2 = (A_2, G_2)$ be two contracts. The composition $\mathcal{C}=(A,G)=\mathcal{C}_1  \parallel  \mathcal{C}_2$ can be computed as follows:
\begin{align}
 A & = (A_1 \cap A_2) \cup \overline{(G_1 \cap G_2)}, \label{eq:sat_composition_A}\\
 G & = G_1 \cap G_2. \label{eq:sat_composition_G}
\end{align}
Intuitively, an implementation satisfying $\mathcal{C}$ must satisfy the guarantees of both $\mathcal{C}_1$ and $\mathcal{C}_2$, hence the operation of intersection in~\eqref{eq:sat_composition_G}.
An environment for $\mathcal{C}$ should also satisfy all the assumptions, motivating the conjunction of $A_1$ and $A_2$ in~\eqref{eq:sat_composition_A}. However, part of the  assumptions in $\mathcal{C}_1$ may be already supported by $\mathcal{C}_2$ and \emph{vice versa}. This allows relaxing $A_1 \cap A_2$ with the complement of the guarantees of $\mathcal{C}$~\cite{benveniste2018contracts}.

\subsubsection{Contract Conjunction}

Different contracts on a single implementation can be combined using the conjunction operation ($\land$). 
Let $\mathcal{C}_1 = (A_1, G_1)$ and $\mathcal{C}_2 = (A_2, G_2)$ be two contracts. We can compute their conjunction by taking the greatest lower bound of $\mathcal{C}_1$ and $\mathcal{C}_2$ with respect to the reﬁnement relation. Intuitively, the conjunction $\mathcal{C}=\mathcal{C}_1  \land  \mathcal{C}_2$ is the weakest (most general) contract that refines both $\mathcal{C}_1$ and $\mathcal{C}_2$. Contract $\mathcal{C}$ can be computed by taking the intersection of the guarantees and the union of the assumptions, that is:
\begin{equation*}
 \mathcal{C} = (A_1 \cup A_2, G_1 \cap G_2).
\end{equation*}
An implementation satisfying $\mathcal{C}$ must satisfy the guarantees of both $\mathcal{C}_1$ and $\mathcal{C}_2$, while being able to operate in either of the environments of $\mathcal{C}_1$ or $\mathcal{C}_2$. 

\subsection{Linear Temporal Logic}
\label{sec:ltl}

Given a set of atomic propositions $\mathcal{AP}$, which are Boolean statements over system variables, we define the satisfaction of a proposition $p \in \mathcal{AP}$ by a state $s$ of a system (a specific valuation of the system variables) as $s \models p$, if $p$ is \textit{true} in state $s$.
LTL formulas over $\mathcal{AP}$ are constructed using the following grammar:
\begin{align*}
    \varphi := p ~|~ \neg\varphi ~|~ \varphi_1 \lor \varphi_2 ~|~ \textbf{X} ~\varphi ~|~ \varphi_1 ~\textbf{U}~ \varphi_2,
\end{align*}
where $\varphi$, $\varphi_1$, and $\varphi_2$ are LTL formulas.
Conjunction ($\land$), implication ($\rightarrow$), and equivalence ($\leftrightarrow$) are definable from negation ($\neg$) and disjunction ($\lor$). Boolean constants \textit{true} and \textit{false} are defined as $\textit{true} = \varphi \lor \neg \varphi$ and $\textit{false} = \neg \textit{true}$, respectively. 
The temporal operators $\textbf{X}$ (next) and $\textbf{U}$ (until) allow us to express temporal properties. Additionally, the operators \textit{globally} ($\textbf{G}$) and \textit{eventually} ($\textbf{F}$) are derived as $\textbf{F}~ \varphi = \textit{true} ~\textbf{U}~ \varphi$ and $\textbf{G} ~ \varphi = \neg(\textbf{F}(\neg \varphi))$.
For the formal semantics of LTL, we refer the reader to the literature~\cite{baier2008principles}.

    Both assumptions and guarantees within a contract can be expressed as LTL formulas. In this case, a contract becomes a pair of LTL specifications, one for the assumptions and one for the guarantees.

\subsection{Reactive Synthesis}
\label{sec:reactive_synthesis}

Reactive synthesis is the process of automatically generating a controller, modeled as a finite state machine, from an LTL specification that distinguishes between inputs and outputs. When a controller, satisfying the specification for all possible inputs, is synthesizable, it guarantees the desired system behavior.

Given an LTL formula $\varphi$ over the atomic propositions $\mathcal{AP}$, partitioned into inputs $\mathcal{I}$ and outputs $\mathcal{O}$ such that $\mathcal{AP} = \mathcal{I} \cup \mathcal{O}$, the synthesis problem is to find a finite-state machine $\Machine$, such as a Mealy machine, that realizes $\varphi$.

A Mealy machine $\Machine$ is defined as a tuple $(S, \mathcal{I}, \mathcal{O}, s_0, \delta)$, where $S$ is a set of states, $s_0 \in S$ is the initial state, and $\delta: S \times 2^\mathcal{I} \rightarrow S \times 2^\mathcal{O}$ is the transition function. A word $w = (w_0^{\mathcal{I}}, w_0^{\mathcal{O}})(w_1^{\mathcal{I}}, w_1^{\mathcal{O}})(w_2^{\mathcal{I}}, w_2^{\mathcal{O}})... \in (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega$ is a \textit{trace} of $\Machine$ if there is a corresponding run $\tau = \tau_0\tau_1\tau_2... \in S^\omega$ with $\tau_0 = s_0$, and for every $i \in \mathbb{N}$, $(\tau_{i+1}, w_i^{\mathcal{O}}) = \delta(\tau_i, w_i^{\mathcal{I}})$. 
$\Machine$ satisfies $\varphi$ if all traces of $\Machine$ satisfy $\varphi$.

Connecting reactive synthesis with contracts, we say that a Mealy machine, or \textit{component, $\Machine$ is a valid \emph{implementation} of a contract $\mathcal{C}$ if it shares the same variables with $\mathcal{C}$ and all behaviors of $\Machine$ satisfy the guarantees $G$ when constrained by the assumptions $A$. If $\mathcal{C}=(\varphi_A, \varphi_G)$ is a contract of LTL specifications, then we say that $\Machine $satisfies $\mathcal{C} $, denoted $\Machine \models \mathcal{C}$, if $\Machine $satisfies $\varphi_A \rightarrow \varphi_G$.
}


==> Tex/casestudy_old.tex <==

\section{Full example}

\label{sec:casestudy}
In the following, we will illustrate how a designer can use \NAME to model the goals of our running example and produce traces that always satisfy the contextual mission.

\subsection{Orchestration}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/mealy-synch.eps}
  \caption{Synchronization between Timed Automata and Mealy Machines. The red arrows indicate the state of the machines at time $t$, when we have a context switch from context $day$ to $night$. The connected red boxes indicate transitions that happen in parallel.} 
  \label{fig:Mealysynch}
\end{figure*}

\vspace{2mm}
Let us consider the two contexts in our running example: $day$ and $night$. We have two instances of $\textit{S-Automaton}$, namely $\textit{S[day]}$ and $\textit{S[night]}$, and two task controllers $\lambda_d'$ and $\lambda_n'$ that realize the specifications $CT(AC(\textit{day})) = \gamma_d$ and $CT(AC(\textit{night})) = \gamma_n$, respectively. We start by considering the three goals $\mathcal{G}_1$, $\mathcal{G}_2$, and $\mathcal{G}_4$, and leave out $\mathcal{G}_3$, requiring the robot to register a person. 
Figure~\ref{fig:Mealysynch} shows the Mealy machines $\lambda_d'$ and $\lambda_n'$ that realize $\gamma_d$ and $\gamma_n$, which have been modified to accept the ``activation inputs'' $\textbf{a}_d$ and $\textbf{a}_n$.

At any time, only one activation input of $\Lambda^{||}$ is set to \textit{true}, indicating that only one Mealy machine in the composition  $\Lambda^{||}$ is active. The functions executed on the transitions of the $\textit{S-Automaton}$ and $\textit{T-Automaton}$ manage the activation inputs in the following ways:

\begin{itemize}
\item \textbf{activate()} is a function executed by every $\textit{S-Automaton}$ instance. 
It is triggered by an $\textit{S-Automaton}$ transitioning from \textit{idle} to \textit{active} state and activates a task controller $\lambda'_i$. Specifically, any $\textit{S-Automaton}$ instantiated for a context $x_i$ that transitions at time $t$ (i.e., $AC(t) = x_i$) from \textit{idle} to \textit{active} will activate the task controller $\lambda_i'$, which realizes the specification $\gamma_i = CT(x_i)$. In Figure~\ref{fig:Mealysynch}, $\textbf{activate()}$ of $\textit{S[day]}$ sets the activation input of $\lambda_d'$ (i.e., $\textbf{a}_d$) to \textit{true}, while $\textbf{activate()}$ of $\textit{S[night]}$ sets the activation input of $\lambda_n'$ (i.e., $\textbf{a}_n$) to \textit{true}.
\item \textbf{deactivate()} is the opposite of the \textbf{activate()} function, as it sets the activation inputs of the corresponding task controllers to \textit{false}. This function is triggered after a context switch when the \textit{Orchestrator} synchronizes with the active \textit{S-Automaton} that transitions from the \textit{active} to the \textit{idle} state.

\item \textbf{trans\_start()} activates one transition controller for every context switch, such as from $day$ to $night$. However, unlike the task controller, there could be more than one transition controllers for each transition automaton. Each transition controller is responsible for guiding the robot from one location to another. The transition controller that needs to be activated after a context switch depends on \textit{where} the robot is when the context switch happens and where it needs to be under the new context. In the example in Figure~\ref{fig:Mealysynch}, the control has to pass from $\lambda_d'$ to $\lambda_n'$, and the transition controller that needs to be activated depends on the current state of $\lambda_d'$ to $\lambda_n'$ when the context switch occurs.
\item \textbf{trans\_end()} is executed when the transition controller has reached its final state and sets its activation input to \textit{false}.
\end{itemize}
\begin{figure*}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/timeline.eps}
  \caption{Timeline.} 
  \label{fig:timeline}
\end{figure*}
Let us assume that at time $t$ we have a context-switch, $\lambda_n'$ is active in state $0$, and $\lambda_d'$ is inactive in state $0$. Each state corresponds to the last region that has been reached by the robot, i.e., region $r_2$ for $\lambda_d'$ and region $r_4$ for $\lambda_n'$.

\textbf{At time t}, $\textit{S[day]}$ transitions from \textit{active} to \textit{idle}, and $\textit{T[day][night]}$ transitions from \textit{idle} to \textit{active}. \textbf{deactivate()} sets $\textbf{a}_d$ to \textit{false}, and \textbf{trans\_start()} chooses the transition controller that can connect the state $0$ of $\lambda_n'$ to the state $0$ of $\lambda_d'$, as indicated by the \textit{source} and \textit{destination} in Figure~\ref{fig:Mealysynch}. In our example, it sets $\textbf{a}{r_{2}r_{4}}$ to \textit{true}.

\textbf{At time t+1}, $\textit{S[day]}$ and $\textit{S[night]}$ are in the \textit{idle} state, and $\textit{T[day][night]}$ is in the \textit{active} state. The transition controller $k'_{r_2r_4}$ moves from state $2$ to state $3$.

\textbf{At time t+2}, the transition controller $k'_{r_2r_4}$ has reached its final state and 
$\textit{T[day][night]}$ transitions from \textit{active} to \textit{idle} causing \textbf{trans\_end()} to execute and set $\textbf{a}_{r_2r_4}$ to \textit{false}. In the same instance, $\textit{S[night]}$ transitions from \textit{idle} to \textit{active} while \textbf{activate()} sets $\textbf{a}_n$ to \textit{true}.

In the full running example, we consider all four goals $\mathcal{G}_1$, $\mathcal{G}_2$, $\mathcal{G}3$, and $\mathcal{G}4$ combined in the CGG under two scenarios: \textit{1)} $\mathcal{G}{d}$, requiring the robot to greet and register people during the day while patrolling regions $r_1$ and $r_2$, and \textit{2)} $\mathcal{G}{n}$, requiring the robot to greet people during the night while patrolling regions $r_3$ and $r_4$.

Figure~\ref{fig:timeline} shows the timeline of events, where the context switches from $day$ to $night$ after a minimum context time of $t_\text{context}$ time units. The timed automaton synchronizes after every context switch and the $\textit{T-Automata}$ are active for at most $t_\text{trans}$ time units. At the bottom of the figure, we can see the trace of the robot $\mathcal{R}$ defined by its \textit{input-output} relationship.

The output symbols inside \textit{boxes} are part of the trace projections for the specification $\gamma_d$ (i.e., related to the goal $\mathcal{G}{d}$), while the outputs inside \textit{circles} are those for the specification $\gamma_n$ (i.e., related to the goal $\mathcal{G}{n}$). At step $3$, the robot perceives a person ($p$), and while it greets immediately ($g$), the registration ($s$) will be executed at step $11$, that is,  the next time the context $day$ is active \textit{and} the robot has finished the transition period.


==> Tex/cgg_copy.tex <==

\section{The Contract-Based Goal Graph (CGG)}
\label{sec:cgg}

The Contract-Based Goal Graph (CGG) is a structured representation of goals within a robotic mission, organized hierarchically to reflect the relationships and dependencies between different objectives. In this framework, goals are treated as nodes within a graph, and the connections between them are indicative of how they relate to or influence one another. The CGG is specifically designed to facilitate the analysis and synthesis of goal-oriented behavior in complex systems, such as robots operating within dynamic and uncertain environments. Here's a detailed explanation:

A CGG is formally defined as a directed graph $T = (\Upsilon, \Xi)$, where each node $\upsilon \in \Upsilon$ represents a goal and each directed edge $\xi \in \Xi$ signifies a relationship between two goals, which can be of three types: refinement, composition, or conjunction. Refinement represents a hierarchical relationship where a goal is broken down into sub-goals. Composition is used to merge goals into a single, more complex goal that captures the behavior necessary to satisfy all individual goals simultaneously. Conjunction links goals that are to be achieved in parallel, indicating that the robot should satisfy all connected goals concurrently, under the assumption that their contexts do not overlap.

The context-based specification clustering algorithm~\cite{mallozzi2020crome} plays a crucial role in addressing Problem 1 (as outlined in Section~\ref{sec:problem}). This algorithm operates as follows:

\begin{enumerate}
\item \textit{Identify Exclusive Contexts:} The first step is to delineate the mutually exclusive contexts within which the robot operates. These contexts form the basis for clustering goals.
\item \textit{Cluster Goals by Compatibility:} Goals are then grouped into clusters based on their compatibility with each exclusive context. A goal is considered compatible with a context if the conjunction of the goal's context and the cluster's mutually exclusive context is logically satisfiable.
\item \textit{Combine Goals Within Clusters:} Within each cluster, goals are combined using the composition operation. This operation generates a new goal that reflects the behaviors needed to satisfy all goals in the cluster, given that the environment satisfies the combined assumptions.
\item \textit{Connect Clusters:} The new goals produced from the composition within clusters are then connected using the conjunction operation. This step is based on the premise that goals with mutually exclusive contexts can be conjoined because their contexts do not occur simultaneously.
\item \textit{Derive Mission Scenarios:} Each goal resulting from the conjunction operation corresponds to a unique mission scenario, reflecting a specific set of behaviors that the robot must exhibit when the associated context is active.
\end{enumerate}

This CGG structure ultimately helps in automating the decision-making process for the robot, ensuring that it can dynamically adjust its behavior to fulfill the mission's goals, adapting as different contexts become active or inactive over time. The CGG not only aids in the clear representation of complex missions but also serves as a foundation for algorithms that synthesize robot behaviors that are robust to changes in the environment.

\subsection{Example}

In our running example, we define four goals and two mission contexts, $X=\{\texttt{day}, \texttt{night}\}$. 
For clarity, we provide name, description, context, assumptions, and guarantees for each goal, denoted by $N, D, ctx, A, G$, respectively. We use $\mathcal{G}_i$ and $\mathcal{C}_i$, with $i \in \{1, \ldots, 4\}$, to denote a goal and its contract. For each contract $\mathcal{C}_i$, we use $\psi_i$ and $\phi_i$ to denote the assumption and guarantee formulas, respectively. 

We associate each region on the map with an atomic proposition in  $\{r_1, r_2, r_3, r_4, r_5\}$. When a region is visited, the corresponding atomic proposition is set to \textit{true}. The actions \textit{greet} and \textit{register} are represented by the atomic propositions $g$ and $s$, respectively. We use $p$ to denote the presence of a \textit{person}. The goal contexts $\texttt{day}$ and $\texttt{night}$ are defined such that $\texttt{day} = \overline{\texttt{night}}$ at all times, i.e., $\texttt{day}$ is the negation of $\texttt{night}$.

\begin{align}
  \mathcal{G}_{1} &=
    \begin{cases}
      N & day\_patrolling\\
      D & \text{Keep visiting regions $r_1$ and $r_2$ in order.}\\
      ctx & \texttt{day}\\
      & \mathcal{C}_{1}
      \begin{cases}
        \psi_1 & true\\
        \phi_1 & \textbf{OP}(r_1, r_2)
      \end{cases}\\
    \end{cases} \notag\\
  \mathcal{G}_{2} &=
    \begin{cases}
      N & night\_patrolling\\
      D & \text{Keep visiting regions $r_3$ and $r_4$ in order.}\\
      ctx & \texttt{night}\\
      & \mathcal{C}_{2}
      \begin{cases}
        \psi_2 & true\\
        \phi_2 & \textbf{OP}(r_3, r_4)
      \end{cases}\\
    \end{cases} \notag\\
  \mathcal{G}_{3} &=
    \begin{cases}
      N & day\_register\\
      D & \text{Register a person promptly after being detected.}\\
      ctx & \texttt{day}\\
      & 
\mathcal{C}_{3}
      \begin{cases}
        \psi_3 & \textbf{AE}(p)\\
        \phi_3 & \textbf{BD}(p, s)
      \end{cases}\\
    \end{cases} \notag \\
    \mathcal{G}_{4} &=
    \begin{cases}
      N & always\_greet\\
      D & \text{Greet a person immediately when detected.}\\
      ctx & true\\
      & \mathcal{C}_{4}
      \begin{cases}
        \psi_4 & \textbf{AE}(p)\\
        \phi_4 & \textbf{IR}(p, g)
      \end{cases}\\
    \end{cases} \notag
\end{align}

\noindent The assumptions $\psi_1$ and $\psi_2$ are set to `true', indicating that these goals do not rely on specific environmental conditions and are always relevant during their respective contexts (\texttt{day} and \texttt{night}). This design choice reflects the ongoing nature of patrolling tasks regardless of additional environmental factors.

\noindent\textbf{AE} (\textbf{AlwaysEventually}) and \textbf{OP} (\textbf{OrderedPatrolling}) are LTL constructs that are key to our example. \textbf{AE} represents the concept of something occurring infinitely often in the future (denoted by $\mathsf{GF}$ in LTL), ensuring ongoing vigilance for certain conditions like the presence of a person. \textbf{OP} is a pattern for periodic visitation of locations in a specified order, crucial for systematic patrolling. For instance, $\textbf{OP}(r_1, r_2)$ ensures that regions $r_1$ and $r_2$ are visited repeatedly in that order. 

\noindent Figure~\ref{fig:example-cgg-controllers} illustrates the CGG for our example, visually depicting the hierarchical structure and interrelationships between the goals and their contexts. This figure aids in understanding how different goals are clustered and combined based on their contexts.

\begin{align*}
  & \mathsf{G} \mathsf{F} (r_{1} ~~\land~~ \mathsf{F} r_{2}) ~~\land~~ (\overline{r_{2}} ~~\mathbin{\mathsf{U}}~~ r_{1}) ~~\land~~ \\
  & \land~~ \mathsf{G} (r_{2} \rightarrow \mathsf{X} (\overline{r_{2}} ~~\mathbin{\mathsf{U}}~~ r_{1})) ~~\land~~ \mathsf{G} (r_{1} \rightarrow \mathsf{X} (\overline{r_{1}} ~~\mathbin{\mathsf{U}}~~ r_{2}))
\end{align*}

\noindent The context $\texttt{day}$ is associated with the cluster $\{\mathcal{G}_1, \mathcal{G}_3, \mathcal{G}_4\}$, while $\texttt{night}$ is linked to  $\{\mathcal{G}_2, \mathcal{G}_4\}$. $\mathcal{G}_4$ appears in both clusters because its context is universally applicable (\textit{true}), making it compatible with any other goal context. This compatibility illustrates how goals can be relevant in multiple mission contexts based on their defined conditions.

\noindent The contracts $\gamma_d$ and $\gamma_n$ result from the composition of the individual goal contracts. They encapsulate the combined requirements for the robot's behavior in both \texttt{day} and \texttt{night} contexts, respectively. This composition ensures that the robot meets all necessary objectives under each context, while respecting the individual constraints of each goal.

\noindent Controllers $\lambda_d$ and $\lambda_n$ are synthesized to manage the robot's behavior for the \texttt{day} and \texttt{night} contexts, respectively. These controllers must be context-aware to handle transitions between the two contexts seamlessly. The robot will switch from $\lambda_d$ to $\lambda_n$ when the context changes from \texttt{day} to \texttt{night}, and vice versa. This dynamic switching allows the robot to adapt its behavior to the active context, ensuring


==> Tex/cgg_orig.tex <==

 \section{The Contract-Based Goal Graph (CGG)}
 \label{sec:cgg}

 The Contract-based Goal Graph (CGG) is a formal model that hierarchically represents goals, where each goal is a node and  nodes can be linked by different relationships. Formally, a CGG is defined as a graph $T = (\Upsilon,\Xi)$, where each node $\upsilon \in \Upsilon$ is a goal and each directed edge $\xi \in \Xi$ is a link that connects two goals. There are three kinds of links: refinement, composition, and conjunction. 

 Given a CGG, we introduce a context-based specification clustering algorithm \cite{mallozzi2020crome} which addresses Problem 1 in Section~\ref{sec:problem}. The algorithm first identifies mutually exclusive goal contexts. It then creates clusters by grouping goals that are \textit{compatible} with each mutually exclusive mission context (compatible means that the conjunction of the goal context with the mutually exclusive context of the cluster is satisfiable).
 Goals may participate in multiple clusters if their context is compatible with the context of the cluster. The goals of each cluster are combined using the \textit{composition} operation, which produces a new goal for each cluster. Finally, the newly produced goals are combined using the \textit{conjunction} operation, since goals having mutually exclusive contexts can be combined with conjnction (as we have see in section ... conjucntion among goal entails the disjunciton of their contexts).
 Each composition produces a new goal that operates in environments that satisfy the assumptions of all the composing goals. On the other hand, the conjunction requires that the resulting goal operate in environments that satisfy at least one of the assumptions of the originating goals. Therefore, composition combines goals within each cluster, while conjunction connects goals with mutually exclusive contexts.
 
 Once the CGG is built, we say that 
 there is one mission scenario for each goal in the conjunction. 
 For instance, suppose there is a mission that has two contexts, $x_1$ and $x_2$, and two goals, $\mathcal{G}_1$ and $\mathcal{G}_2$, operating under mutually exclusive Boolean formulas, $ctx_1$ and $ctx_2$, respectively, that are satisfiable with $x_1$ and $x_2$.
 
\subsection{Example}

In our running example, we define four goals and two mission contexts, $X=\{\texttt{day}, \texttt{night}\}$. 
For clarity, we provide name, description, context, assumptions, and guarantees for each goal, denoted by $N, D, ctx, A, G$, respectively. We use $\mathcal{G}_i$ and $\mathcal{C}_i$, with $i \in \{1, \ldots, 4\}$, to denote a goal and its contract. For each contract $\mathcal{C}_i$, we use $\psi_i$ and $\phi_i$ to denote the assumption and guarantee formulas, respectively. \pierl{Can we simplify further since there is redundancy in the way we denote assumptions and guarantees. This is not good notation.}

We associate each region on the map with an atomic proposition in  $\{r_1, r_2, r_3, r_4, r_5\}$. When a region is visited, the corresponding atomic proposition is set to \textit{true}. The actions \textit{greet} and \textit{register} are represented by the atomic propositions $g$ and $s$, respectively. We use $p$ to denote the presence of a \textit{person}. The goal contexts $\texttt{day}$ and $\texttt{night}$ are defined such that $\texttt{day} = \overline{\texttt{night}}$ at all times, i.e., $\texttt{day}$ is the negation of $\texttt{night}$.

\begin{align}
  \mathcal{G}_{1} &=
    \begin{cases}
      N & day\_patrolling\\
      D & \text{Keep visiting regions $r_1$ and $r_2$ in order.}\\
      ctx & \texttt{day}\\
      & \mathcal{C}_{1}
      \begin{cases}
        \psi_1 & true\\
        \phi_1 & \textbf{OP}(r_1, r_2)
      \end{cases}\\
    \end{cases} \notag\\
  \mathcal{G}_{2} &=
    \begin{cases}
      N & night\_patrolling\\
      D & \text{Keep visiting regions $r_3$ and $r_4$ in order.}\\
      ctx & \texttt{night}\\
      & \mathcal{C}_{2}
      \begin{cases}
        \psi_2 & true\\
        \phi_2 & \textbf{OP}(r_3, r_4)
      \end{cases}\\
    \end{cases} \notag\\
  \mathcal{G}_{3} &=
    \begin{cases}
      N & day\_register\\
      D & \text{Register a person promptly after being detected.}\\
      ctx & \texttt{day}\\
      & 
\mathcal{C}_{3}
      \begin{cases}
        \psi_3 & \textbf{AE}(p)\\
        \phi_3 & \textbf{BD}(p, s)
      \end{cases}\\
    \end{cases} \notag \\
    \mathcal{G}_{4} &=
    \begin{cases}
      N & always\_greet\\
      D & \text{Greet a person immediately when detected.}\\
      ctx & true\\
      & \mathcal{C}_{4}
      \begin{cases}
        \psi_4 & \textbf{AE}(p)\\
        \phi_4 & \textbf{IR}(p, g)
      \end{cases}\\
    \end{cases} \notag
\end{align}
\nir{Why is $AE(p)$ needed in $G_3$ and $G_4$?}
\pierg{otherwise the the environment wins by never setting $p$}

\noindent\textbf{AE} (\textbf{AlwaysEventually}) represents the LTL construct globally eventually ($\mathsf{GF}$). \textbf{OP} ($\textbf{OrderedPatrolling}$) is a robotic pattern that expresses the periodic visit of a set of locations in a given order. For example, $\textbf{OP}(r_1, r_2)$ corresponds to the LTL formula:
\begin{align*}
    & \mathsf{G} \mathsf{F} (r_{1} ~~\land~~ \mathsf{F} r_{2}) ~~\land~~ (\overline{r_{2}} ~~\mathbin{\mathsf{U}}~~ r_{1}) ~~\land~~ \\
    & \land~~ \mathsf{G} (r_{2} \rightarrow \mathsf{X} (\overline{r_{2}} ~~\mathbin{\mathsf{U}}~~ r_{1})) ~~\land~~ \mathsf{G} (r_{1} \rightarrow \mathsf{X} (\overline{r_{1}} ~~\mathbin{\mathsf{U}}~~ r_{2}))
\end{align*}
Finally, $\textbf{BD}$ (\textbf{BoundDelay}) and $\textbf{IR}$ (\textbf{InstantaneousReaction}) are robotic patterns which require an action \textit{a} (i.e., setting a proposition to \textit{true}) based on the truth value of an atomic proposition $s$. They correspond to the LTL formulas $\mathsf{G}(s \leftrightarrow a)$ and $\mathsf{G}(s \rightarrow a)$, respectively. For more details and the complete list of robotic patterns, see Menghi et al.~\cite{patterns}. 

\begin{figure}
  \centering
  \includegraphics[width=0.8\columnwidth]{figures/example-cgg-controllers.eps}
  \caption{CGG created for the running example.}
  \label{fig:example-cgg-controllers}
 \end{figure}

Given $\mathcal{G}_1$, $\mathcal{G}_2$, $\mathcal{G}_3$, and $\mathcal{G}_4$, the context-based specification clustering algorithm of \NAME produces two mutually exclusive goal contexts, namely, \texttt{day} and \texttt{night}. The context $\texttt{day}$ is associated with the cluster $\{\mathcal{G}_1, \mathcal{G}_3, \mathcal{G}_4\}$, while $\texttt{night}$ is linked to  $\{\mathcal{G}_2, \mathcal{G}_4\}$. $\mathcal{G}_4$ is present in both clusters since its context (\textit{true}) is compatible with any goal context. \pierl{to be formalized better early on}

Figure~\ref{fig:example-cgg-controllers} shows the CGG produced by \NAME, where $\mathcal{G}{d}$ is the goal resulting from the composition of goals $\mathcal{G}{1}$, $\mathcal{G}{3}$, and $\mathcal{G}{4}$ with the following contract: \pierl{I think it is really not good to introduce this strange notion of composition here}
\begin{align}
  \mathcal{C}_{d} &=
      \begin{cases}
        \psi_d & \textbf{AE}(p) \lor \overline{\phi_d} \\
        \phi_d & \textbf{OP}(r_1, r_2) \land (\mathsf{GF}(p) \rightarrow \textbf{BD}(p, s))
      \end{cases}\notag
\end{align}
\pierl{I don't understand where this contract is coming from.}
$\mathcal{G}_{n}$ is the composition of goals $\mathcal{G}_{2}$ with $\mathcal{G}_{4}$ and has the following contract:
\begin{align}
  \mathcal{C}_{n} &=
      \begin{cases}
        \psi_n & \textbf{AE}(p) \lor \overline{\phi_n} \\
        \phi_n & \textbf{OP}(r_3, r_4) \land (\textbf{AE}(p) \rightarrow \textbf{IR}(p, g))
      \end{cases}\notag
\end{align}
We now compute the two mission scenarios for the two mission contexts $X=\{\texttt{day}, \texttt{night}\}$. We have that $\mathcal{M}_d = (\texttt{day}, \gamma_d)$ and $\mathcal{M}_n = (\texttt{night}, \gamma_n)$, where $\gamma_d$ and $\gamma_n$ are produced from the contracts $\mathcal{C}_{d}$ and $\mathcal{C}_{n}$ as follows:
\begin{align}
  \gamma_d &= \psi_{d} \rightarrow \phi_{d} \label{spec:gamma2}\\
  \gamma_n &= \psi_{n} \rightarrow \phi_{n} \label{spec:gamma1}
\end{align}
\pierl{Skip the implication formulas and leave just the contracts in the scenarios.}

We can generate two controllers, $\lambda_d$ and $\lambda_n$, via reactive synthesis from the contracts $\gamma_d$ and $\gamma_n$, respectively \pierl{Please introduce contracts then}. However, these controllers are agnostic to the context. To satisfy the contextual mission, we need the robot to switch from $\lambda_d$ to $\lambda_n$ when the context changes from $\texttt{day}$ to $\texttt{night}$. Additionally, we want the robot to switch back to $\lambda_d$ and resume or complete its task when $\texttt{day}$ becomes true again, i.e., when $\mathcal{M}_{d}$ is the active scenario. In the following, we detail a method to produce robot behaviors that ensure mission satisfaction in the presence of context changes.

\nir{ 
The idea of context state formulas and the way they are done in the contracts results in a very strange behaviour.
}
\nir{
Consider a circling behaviour that is defined under the context state formula true.
Circle between r1 r2 r3 r4 in this order. However, because it is true for multiple contexts the circling will restart and hold distance cycles PER CONTEXT.
}
\pierg{i dont follow this}
\nir{
I think that this should be removed (along with all the contract surrounding it, but if you insist to push the contract approach I won't object. But not in this strange way).
}\pierg{let's keep it, contract in general add value but it could be that in this particular case of synthesis the result is the same} \pierl{I totally agree with Nir. Contracts can add value in compositional verification and synthesis. However, the way they are introduced here, especially in this writeup, seems really strange and needs careful rethinking and reformulation.}



==> Tex/conclusions_old.tex <==

\section{Conclusions}
\label{sec:conclusion}

This paper presents a design framework for capturing and formalizing robotic requirements for contextual missions, with a focus on realizing modular and efficient mission controllers. We introduce \NAME, a tool that uses specification patterns and contexts to translate informal requirements into formal goals. These goals are then transformed into assume-guarantee contracts and organized in a formal model called the contract-based goal graph (CGG). In addition, we address the challenge of dynamically switching controllers for different mission scenarios, where each scenario is activated under a mutually exclusive context. To synthesize the overall contextual mission specification, we utilize \CROME to analyze, produce, and orchestrate several controllers.
Our results show that our approach can produce a leaner and more modular specification, which greatly improves synthesis time. In the future, we plan to extend our approach by exploring a new logic language to express the class of problems addressed in this paper. Finally, we intend to validate our approach with larger industrial case studies.



==> Tex/discussion.tex <==

\section{Mission satisfaction and CGG satisfaction Relationship}
\label{sec:missionvscgg}
In Theorem~\ref{thm:missionsatisfaction} we proved that the robot behavior produced by \NAME satisfies the contextual mission. However, such behavior could \textit{not} satisfy the mission as specified in the root of the CGG, which is not a problem as we never required that. However, we could still be interested in having in the root node of the CGG a specification that represents an \textit{abstraction} of the behavior generated by the orchestration system.

Let $\mathcal{C} = (\psi, \phi)$ be the contract formalizing the root goal of the CGG $\mathcal{G}$ which is produced by the conjunction of all the mission scenarios. Each mission scenarios is built from specifications that do not contain the notion of context while the final robot behavior is produced by the orchestration of different controllers according to \textit{1)} the context and \textit{2)} the transition of the robot from one context to another. It can happen that, according to the robotic pattern chosen by the designer to model the different goals, the robot behavior while satisfying the mission does not satisfy the specification in the CGG.

For example, in our running example we have the goal $\mathcal{G}_r$ formalized by the trigger pattern $BoundedReaction$ which performs the counteraction (i.e. $register$) in the \textit{next} time instant, every time and only when the pre-condition (i.e. $person$) is true. This goal is expressed in LTL as
\begin{equation}
\label{eq:personeregister}
    \textbf{G}(person \leftrightarrow \textbf{X} register)
\end{equation} 
However, if we consider the example in Figure~\ref{fig:timeline}, since a person is detected at $t=3$ in order to satisfy (\ref{eq:personeregister}) $\mathcal{R}$ would need to set $register$ to true when $t=4$, but since the context changes at $t=4$ it will satisfy the postcondition only the \textit{next} time when the $day$ context is true and $\mathcal{R}$ is not transitioning, i.e. $t=11$.

Such problems only happen with the \textit{`avoindance'} and \textit{`trigger'} patterns of the robotic catalog~\cite{menghitse}. The \textit{`core movement'} patterns (e.g. \textit{patrolling} a set of locations $\textbf{G}(\textbf{F}(r_1, r_2,...r_n))$ or \textit{`visit'} patterns (e.g. $\textbf{F}(r_1, r_2,...r_n)$) are not affected by the context-switch since they only indicate the order in which location specified must be visited; they do not forbid to visit other locations. However we have to assume that the set of regions refer by each mission scenario is disjoint.

\begin{definition}[Disjoint scenarios]
    \label{def:disjointscenarios}
    Let $\mathcal{AP}^i_r \subseteq \mathcal{AP}_r$ be the subset of atomic propositions referring to region variables in the specification $\gamma_i \in \Gamma$. Then for any $\gamma_i, \gamma_j  \in \Gamma$ where $i \neq j$ if $\mathcal{AP}^i_r \cap \mathcal{AP}^j_r = \emptyset$ then we say that we have \textit{disjoint scenarios}.
\end{definition}

\begin{remark}
    \ins{The orchestration system of \CROME will order the location to be visited according to the context while satisfying the original pattern formulation.
    Since each context is mutually exclusive, assuming that we have disjoint scenarios (\ref{def:disjointscenarios}), then as long as the order of visit or patrolling is kept, then any trace of $\mathcal{R}$ also satisfies the conjunction of the mission scenarios, i.e., the root node of the CGG.}
\end{remark}

We have the robotic patterns so that the contract at the root of the CGG includes all the behaviors produced by \CROME.
We define a boolean variable $c_i=x_i \land Active$ for any context $x_i \in X$ and where $Active \in \mathcal{O}$ is the active Boolean signal of $\mathcal{R}$ determining when the robot is \textit{not} transitioning from one specification to another. In the following, we show the modified patterns together with their original version:

\begin{align*}
    \textit{Instant Reaction}~~~ &\textbf{G}(p_1 \rightarrow p_2)\\
    \text{modified with}~~~ &\textbf{G}((p_1 \land c_i) \rightarrow (p_2 \land c_i))
\end{align*}

\begin{align*}
    \textit{Delayed Reaction}~~~ &\textbf{G}(p_1 \rightarrow \textbf{F}(p_2))\\
    \text{modified with}~~~ &\textbf{G}((p_1 \land c_i) \rightarrow \textbf{F}(p_2 \land c_i))
\end{align*}

\begin{align*}
    \textit{Prompt Reaction}~~~ &\textbf{G}(p_1 \rightarrow \textbf{X}(p_2))\\
    \text{modified with}~~~ &\textbf{G}((p_1 \land c_i) \rightarrow \textbf{X}(\neg c_i \textbf{W} (p_2 \land c_i)))
\end{align*}

\begin{align*}
    \textit{Bound Reaction}~~~ &\textbf{G}(p_1 \leftrightarrow p_2)\\
    \text{modified with}~~~ &\textbf{G}((p_1 \land c_i) \leftrightarrow (p_2 \land c_i))
\end{align*}

\begin{align*}
    \textit{Bound Delay}~~~ &\textbf{G}(p_1 \leftrightarrow \textbf{F}(p_2))\\
    \text{modified with}~~~ &\textbf{G}((p_1 \land c_i) \leftrightarrow \textbf{X}(\neg c_i \textbf{W} (p_2 \land c_i)))
\end{align*}

\begin{align*}
    \textit{Wait}~~~ &r_1 \textbf{U} p_3\\
    \text{modified with}~~~ & ((r_1 \land c_i) \lor \neg c_i) \textbf{U} (p_1 \land c_i)
\end{align*}

Where $p_1 \in \{S \cup R \cup A$\}, $p_2 \in \{R \cup A$\}, $p_2 \in \{S \cup A$\} and $r_1 \in R$.

\begin{remark}
    Realizing the specification directly with the modified patterns does not produce a controller that satisfies the mission since the modifications were only applied to some of the patterns and the behavior of $Active$ variable is not always specified.
\end{remark}
    


==> Tex/evaluation_old.tex <==
\section{Implementation}\label{sec:implementation}
\NAME is implemented as a web-based tool and is available open source\footnote{\NAME tool: \url{rebrand.ly/crometool}}. The tool utilizes NuXMV~\cite{nuxmv} and STRIX~\cite{strix} as back-end engines to check the satisfiability and realizability of the specifications, respectively. After building the CGG, each mission scenario is realized in a task controller, i.e., a Mealy machine.

Concerning the realization of the transition controller, there are two main factors to consider. A first factor is the number of location pairs. Depending on the mission specifications, certain context switches may require the robot to move to a different set of locations. Assuming the worst-case scenario, where all context switches require a change in location, we can define the set of regions $R$ as the union of mutually exclusive sets of regions $\Omega_{R1}, \Omega_{R2},..., \Omega_{Rn}$ activated by context variables $x_1, x_2,...,x_n$. In this case, the total number of location pairs that require a transition controller is $(|\Omega_{R1}| \times |\Omega_{R2}| \times ... \times |\Omega_{Rn}|) \times 2$, taking into account all possible pairs of locations and their permutations.

The second factor is the generation of the transition controller. Given the map of the environment, the task of generating a transition controller is essentially a shortest path problem. Although \NAME uses reactive synthesis to produce the transition controller, any algorithm that solves the shortest path problem (such as Dijkstra) could be used instead.

In our example, we may need up to eight transition controllers, four for each direction between regions operating under the \textit{day} and \textit{night} contexts. However, \NAME uses an algorithm that considers the environment map and adjacent locations to minimize the number of controllers generated. For instance, in Figure~\ref{fig:illustrative}, the algorithm only generates one controller that leads to location $r_5$. Since $r_5$ is adjacent to all other locations, the robot can reach any location by going to $r_5$.

A simple algorithm for generating transition controllers is to find a path from the \textit{source} location to the \textit{destination} location that satisfies the transition time constraint, i.e., no more than $t_{\texttt{trans}}$ steps. The algorithm tries paths of length $1<N<t_{\texttt{trans}}$ until it finds one that satisfies the constraint. However, \NAME implements a more sophisticated algorithm that considers the map of the environment and adjacent locations to reduce the number of controllers needed.

\section{Evaluation}
\label{sec:evaluation}

\newcommand\mstime{$35.6~$}

\newcommand\msstates{$119~$}
\newcommand\mstransitions{$357~$}
\newcommand\cstime{$0.14~$}
\newcommand\csstates{$5 ~\text{and}~ 3~$}
\newcommand\cstransitions{$~10 ~\text{and}~ 6~$}

\newcommand\nttrans{$16~$}
\newcommand\talltrans{$0.92~$}
\newcommand\cggtime{$0.54~$}
\newcommand\totaltime{$1.60~$}

\newcommand\cfaster{$254~$ times}
\newcommand\cfastermod{$22~$ times}

\begin{table}[t]
{\small
    \begin{TAB}(r,1cm,1cm)[5pt]{|r|c|c|}{|c|c|c|c|}
        & Monolithic LTL  & \NAME \\
        Synthesis Time (sec) & \mstime & \cstime \\
        Number of States & \msstates & \csstates \\
        Number of Transitions & \mstransitions & \cstransitions
    \end{TAB}    
    \caption{Comparison of \NAME with the synthesis from a single LTL formula in order to realize the running example.}
    \label{tab:evaluation}
    }
\end{table}

We evaluated our approach by measuring the synthesis time required by \NAME to generate traces that satisfy the robotic mission in the running example. As our running example is relatively small, we were able to produce a `monolithic' LTL specification that expressed all the desired behaviors and constraints of the contextual mission. We added extra variables to keep track of the context, active signal, and transition conditions from one context to another. Furthermore, we needed an additional Boolean variable for any state where robot execution can halt due to a context switch. This remarkably increased the size of the LTL formula. The full monolithic LTL specification and the test conducted can be found online\footnote{\NAME evaluation: \url{rebrand.ly/cromeevaluation}}. We report the results of the comparison below.

Table~\ref{tab:evaluation} displays the synthesis time and the size of the controller produced by the two approaches, monolithic LTL vs. \NAME. The monolithic LTL formula took \mstime seconds to synthesize, producing a controller having \msstates states and \mstransitions transitions. On the other hand, \NAME, thanks to its lean and modular approach, only had to synthesize the controllers for the two mutually exclusive contexts: $day$ and $night$. Specifically, it had to synthesize the specification $\gamma_1$ (see formula (\ref{spec:gamma1})) related to the goal $\mathcal{G}{ng}$ and the specification $\gamma_2$ (see formula (\ref{spec:gamma2})) related to the goal $\mathcal{G}{dgr}$. These specifications are much smaller, and it only took \cstime seconds to synthesize both of them, which is \cfaster\ faster than the monolithic synthesis. The controllers produced for the two scenarios consist of only \csstates states and \cstransitions transitions, respectively.

Table~\ref{tab:evaluation} does not include the time to generate the transition controllers, as these can be generated using several algorithms. The time taken by \NAME to realize all the transition controllers via reactive synthesis is \talltrans seconds. Additionally, we should take into account that the specifications $\gamma_1$ and $\gamma_2$ are not given directly by the designer, but are produced by \NAME during the creation of the CGG. To produce $\gamma_1$ and $\gamma_2$ from a set of the four input goals provided by the designer, \NAME performed 11 satisfiability checks and 10 validity checks. The creation of the CGG took a total of \cggtime seconds.

Finally, considering the time needed to produce the CGG and all 16 transition controllers, the total synthesis time is \totaltime seconds, which is still a \cfastermod{} improvement compared to synthesizing the monolithic LTL specification.



==> Tex/implementation.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/uml}
  \caption{Main classes composing the \NAME framework}
  \label{fig:uml}
\end{figure*}

\section{\NAME framework}
\label{sec:framework}

Figure~\ref{fig:uml} shows the main classes composing our framework. To model mission requirements and produce a mission specification, the designer can model the environment as a \textit{World}, which is composed by a set of instances of \textit{Type} elements related to each other in a \textit{Typeset} and modeling \text{sensors}, \text{locations}, \text{actions}, and \text{context}. The designer can formalize a goal in terms of \textit{Contract} which is composed of two \textit{Specification} elements, one for the \textit{assumptions} and one for the \textit{guarantees}. \pierl{Have we ever introduced a goal and what it is in this paper?} Specifications \pierl{We use this word in many ways, which can become confusing. We talk about mission specification (see second sentence) then the specifications within a contract, etc.} are expressed by temporal logic formulas that can be directly provided by the user or generated from robotic patterns. Every \textit{Contract} is connected to a \textit{Goal}, which represents tasks to be performed by the robot. Finally, goals can be connected with a \textit{Link} of type \textit{composition}, \textit{refinement}, or \textit{conjunction}. \pierl{Are these defined for goals too?} The set of all goals, linked together, forms the \textit{CGG}. In the following, we describe some of the elements of our framework, while in Section~\ref{sec:cgg} we present the CGG. \pierl{I think we should better relate contracts and goals. Did we do this before? Also, it a bit usual to start the description of a framework with the class diagram (how the components are implemented) rather than the formal definition of the different components of the framework (what the components are)? I assume you cover this in the subsection?} \pierg{Yes i don't want to be too repetitive, the relation between goals and contract is formalized with the UML model, and described in this section. Also in the 'Goal' subsection we say that 'We reduce all the formal operations, checks, and comparisons among goals to their corresponding contracts.'. I think is good to say it there, and not in the 'cappa' of the section?}

\subsection{\textbf{Type}}
A \textit{Type} represents a variable domain. The basic types supported are \textit{Boolean} and \textit{BoundedInteger}. By extending the basic types, \NAME builds more refined ones such as \textit{BooleanAction}, \textit{BooleanLocation}, and \textit{IntegerSensor}, representing  variables indicating actions, physical locations, and sensors withing a certain range, respectively. 
Each type has a \textit{TypeKind} that can be one of the following: \textit{sensor}, \textit{location}, \textit{action} or \textit{context}.

Types derived by extending the basic \textit{Boolean} type can be made mutually exclusive among each other by indicating for each type what \textit{mutex groups} it belongs to. A \texttt{mutex\_group is a \textit{string} and }instances of types belonging to the same \texttt{mutex\_group} can never evaluate to $true$ at the same time. For example, let $A, B,$ and $C$ be three types extending  \textit{BooleanAction and $mtx'$ and $mtx''$ be two mutex groups. $A$ belongs to $mtx'$, $B$ belongs to $mtx''$ and $C$ belongs to both $mtx'$ and $mtx''$. In this example $C$ is mutually exclusive with both $A$ and $B$; so, whenever an instance of $C$ is true, then any instance of $A$ and $B$ must be false. When instances of $C$ are false there are no constraints on the value of the instances of $A$ and $B$.} 

Types representing physical locations, which are types derived by extending \textit{BooleanLocation}, can also indicate their \texttt{adjacency\_set}, that is, a set of \textit{locations} that are geographically adjacent. Assuming that a set of geographical locations are mutually exclusive, only one instance is true at any time step. The \texttt{adjacency\_set} indicates which instances are allowed to be true in the \textit{next} time step.

\subsection{\textbf{Typeset}}
A \textit{Typeset} is a set of \textit{Type} elements and the relationships among them.
The attributes \texttt{refinement\_rel}, \\\texttt{mutex\_rel}, and \texttt{adjacency\_rel} in each Typeset keeps track of the \textit{refinement}, \textit{mutually exclusion}, and \textit{adjacency} relationship among the elements in the typeset, respectively. The refinement relationships are defined by the hierarchical structure of the types, i.e., how the designer \textit{extend other types. Similarly the adjacency and mutual exclusion relationships are extracted from the corresponding properties expressed on the types by the designer. } 

\subsection{\textbf{World}}
The \textit{World} is a \textit{Typeset} that exists independently from a certain specification.
In the following, we will indicate the type, i.e., the domain, by capitalizing the first letter, and variables with lowercase letters.
For example, the environment in the running example in Figure~\ref{fig:illustrative} can be formulated as a \textit{World} containing:

\begin{itemize}
    \item $2$ region types $R_t$ and $R_b$ both extending the \textit{BooleanLocation} type and being mutually exclusive on $group1$. These regions represent the top and the bottom part of the environment in Figure~\ref{fig:illustrative} and are instantiated with the variables $r_t$ and $r_b$. \pierl{Do you mean these are variables of different types?}\pierg{yes}
    \item $5$ regions types $\{R_{i} \mid i=1..5\}$ also extending \textit{BooleanLocation} and mutually exclusive on $group2$. We have that $R_1$ and $R_2$ also extend $R_t$ while $R_3$ and $R_4$ extend $R_b$ since they are refinements of the top and bottom regions. We also have that $R_1$ is adjacent to $R_2$ and $R_5$, $R_2$ is adjacent to $R_1$ and $R_5$, and so on. We denote the variables instantiated from these types by $r_1, r_2, r_3, r_4$, and $r_5$.
    \item $2$ types $\{Day$,  $Night\}$, \pierg{Set notation with `and' in between is unusual?}, extending \textit{BooleanContextTime}, which are mutually exclusive on $group3$ and have their variables being $day$ and $night$.
\end{itemize}

\pierl{I get lost in a lot of low-level details about the implementation of the framework, without motivation and appropriate definition. This makes me lose the sense of what is the overall framework and what it is supposed to do.}\pierg{i addressed your comments. The comment on 'specification' is hard to solve because it is indeed used in mutiple cases. but it should be clear from the context. Or how can we fix it?}

\subsection{\textbf{Specification}}

A \emph{specification} represents an LTL formula, which in \NAME can be constructed with a pattern, i.e., a specification pattern or a robotic pattern. 
\gs{Not sure about the intended meaning of the first part of the sentence (I wouldn't say that a specification "represents" an LTL formula). Is the idea to say that instead of writing specifications in LTL we write patterns? We should then be more direct and say that.}\pierg{a specification is the 'Specification' as data structure in the UML model... so it \textit{represents} the LTL ... I put it in quotes...?} \pierl{I agree this part is not clear.}
A pattern can either be an \textit{Atom}, i.e. a single LTL expression that cannot be broken down in smaller chunks, \pierl{what does this mean? An LTL expressions is already a formula. Do you mean an atomic proposition?} or a \textit{Formula}, i.e. a set of atoms connected via conjunction or disjunction. 
Each specification is defined over a Typeset. For example, let us have a Typeset containing two elements: \textit{BooleanSensor} type $s$ and the \textit{BooleanAction} type $a$, both extending the basic Boolean Type.
The robotic pattern \textit{`InstantReaction'} applied to the atomic propositions $s$ and $a$ is an \textit{Atom} representing the LTL formula: 
\begin{equation}
\label{eq:instantreaction}
    \textbf{G}(s \rightarrow a)
\end{equation}
Instead, the robotic pattern \textit{`Visit'} applied to the atomic propositions $r_1$ and $r_2$ (defined over \textit{BooleanLocation} types) is a \textit{Formula} containing the conjunction of two Atom elements and represented by the LTL formula:
\begin{equation}
\label{eq:visit}
    \textbf{F}(r_1) \land \textbf{F}(r_2)
\end{equation}

We will use the same symbol to indicate both the \textit{variable} and the \textit{atomic proposition} associated to the variable. For example, in (\ref{eq:visit}) $r_1$ and $r_2$ are atomic propositions that represent the truth value of corresponding variables.

\subsubsection{Rules}
Additional formulas can be inferred from each specification by checking its Typeset. \NAME automatically infers the following formulas:

\begin{itemize}
    \item \textit{Mutually Exclusion Rules} $\varphi^\text{mtx}$ for any mutually exclusive relationship in the Typeset.
    \item \textit{Refinement Rules} $\varphi^\text{ref}$ for every refinement relationship in the Typeset.
    \item \textit{Adjacency Rules} $\varphi^\text{adj}$ for every adjacency relationship in the Typeset.
\end{itemize}

For example, let us consider the \textit{world} $W$ described in the previous paragraph \pierl{section?} and shown in Figure~\ref{fig:illustrative}.
Let $W=\{r_t, r_b, r_1, r_2, r_3, r_4, r_5, day, night\}$ be its set of types; then, the rules that can be inferred are:

\begin{align}
    \varphi^\text{mtx}_1 &= \textbf{G}( r_b \leftrightarrow \neg r_b )\label{eq:exmutestops}\\
    \varphi^\text{mtx}_2 &= \bigwedge\limits_{i=1, \ldots, 5} \textbf{G}( r_i \leftrightarrow \bigwedge\limits_{i \neq j} \neg r_j )\label{eq:exmutextregions}\\
    \varphi^\text{mtx}_3 &= \textbf{G}( day \leftrightarrow \neg night )\label{eq:exmutextcontext}\\
    \varphi^\text{ref}&= \textbf{G}((r_1 \lor r_2) \rightarrow r_t) \land \textbf{G}((r_3 \lor r_4) \rightarrow r_b)\label{eq:exref}\\
    \varphi^\text{adj} &= \bigwedge\limits_{i=1..5} \textbf{G}(r_i \rightarrow \bigvee\limits_{r' \in Adj(r_i)} \textbf{X} ~({r'}))\label{eq:topology}
\end{align}
where (\ref{eq:exmutestops}), (\ref{eq:exmutextregions}), and (\ref{eq:exmutextcontext}) model the mutually exclusion conditions.
The refinement relationships are modeled in~(\ref{eq:exref}).
Finally, topology is modeled with~(\ref{eq:topology}) where $Adj(r)$ denotes the locations adjacent to $r$ (including $r$ itself).

To represent the requirements of the robot patrolling the locations in a strict order, we could use the robotic specification pattern \textit{StrictOrderedPatrolling} while to perform the actions we could use the \textit{reaction patterns}~\cite{SpecificationPatternsTSE}.
Let $\textbf{OP}$, $\textbf{BR}$ and $\textbf{BD}$ be symbols representing the \textit{StrictOrderedPatrolling}, \textit{BoundRection} and \textit{BoundDelay} robotic patterns, respectively. We can instantiate the patterns using the atomic proposition in our example and defining the set of specifications $\Gamma=\{\gamma_d, \gamma_n, \gamma_g\, \gamma_r\}$ where:
\begin{align}
    \gamma_d &= \textbf{OP}({r_1}, {r_2})\label{eq:gamma1}\\
    \gamma_n &= \textbf{OP}({r_3}, {r_4}) \label{eq:gamma2}\\
    \gamma_g &= \textbf{BD}({person}, {greet})\label{eq:gammagreet}\\
    \gamma_r &= \textbf{BR}({person}, {register}) \label{eq:gammaregister}
\end{align}

\subsubsection{Checks}
Any specification in \NAME must be satisfiable. To check for satisfiability, \NAME takes into consideration the \textit{mutually exclusion rules} of the specification. Validity checks are used to check refinements among specifications, and so they must take into consideration any possible \textit{refinement rules}.
Finally, realizability checks consider all kinds of rules: mutually exclusion, refinement, and adjacency. \pierl{Why?}

\subsubsection{Operations}
A new specification can be created from simpler ones via \textit{conjunction} ($\land$), \textit{disjunction} ($\lor$) and \textit{negation} ($\neg$) of \textit{Formula} and \textit{Atom} elements. In each formula, we keep both the conjunctive (\textit{'cnf'}) and disjunctive (\textit{'dnf'}) normal forms (treating any \textit{Atom} elements as a \textit{literals}). 
For example, a disjunction between the \textit{Atom} in (\ref{eq:instantreaction}) and the \textit{Formula} in (\ref{eq:visit}) would result in the following \textit{Formula} where both the \textit{'dnf'} and \textit{'cnf'} representations are formed by two other \textit{Formula} elements (separated by a comma) as follows:

\begin{align}
    \text{cnf:}~~~ & (\textbf{F}(r_1) \lor \textbf{G}(s \rightarrow a)) &\land~~~~~& (\textbf{F}(l_2) \lor \textbf{G}(s \rightarrow a))\\
    \text{dnf:}~~~ & (\textbf{F}(r_1) \land \textbf{F}(r_2)) &\lor~~~~~& (\textbf{G}(s \rightarrow a))
\end{align} 
A \textit{Formula} can always be represented as the conjunction or disjunction of all the elements in the \textit{cnf} or \textit{dnf} representations, respectively. \pierl{This section is a bit confusing. It uses a terminology that is not formally introduced and can lead to ambiguities.}

\subsubsection{Comparisons}
Specifications can be compared among each other with the operators $\le$, $<$, $==$, $\neq$, $>$, $\ge$, where $<$ and $>$ represent the \textit{refinement} and \textit{abstraction} relationships, respectively. Let $\varphi_1$ and $\varphi_2$ be two specifications, we have that:

\begin{align}
    \varphi_1 &== \varphi_2 &\textbf{iff}~~~~& (\varphi_1 \rightarrow \varphi_2 \land \varphi_2 \rightarrow \varphi_1) ~~ \text{is \textit{valid}}\\
    \varphi_1 &\neq \varphi_2 &\textbf{iff}~~~~& \neg (\varphi_1 == \varphi_2)\\
    \varphi_1 &\leq \varphi_2 &\textbf{iff}~~~~& (\varphi_1 \rightarrow \varphi_2) ~~ \text{is \textit{valid}}\\
    \varphi_1 &\geq \varphi_2 &\textbf{iff}~~~~& (\varphi_2 \rightarrow \varphi_1) ~~ \text{is \textit{valid}}\\
    \varphi_1 &< \varphi_2 &\textbf{iff}~~~~& (\varphi_1 \leq \varphi_2) \land (\varphi_1 \neq \varphi_2)\\
    \varphi_1 &> \varphi_2 &\textbf{iff}~~~~& (\varphi_1 \geq \varphi_2) \land (\varphi_1 \neq \varphi_2)
\end{align}

Every time a check, a comparison, or an operation among specifications is performed, new constraints are extracted from the \textit{Typeset} of each specification involved. Specifically, \NAME creates a new \textit{Typeset} containing the \textit{union} of all the \textit{types} in all the typesets and extracts a new set of refinement, mutually exclusion, and adjacency relationships. 

\subsection{\textbf{Contract}}
A contract $\mathcal{C}=(\psi, \phi)$ is a tuple of specifications, where $\psi$ is the assumptions and $\phi$ is the guarantees. The guarantees in a contract are always considered in their saturated form, i.e. having guarantees $\psi \rightarrow \phi$. If a contract gets its assumptions changed or updated, its guarantees will change as well due to saturation.

For our running example, we can formalize three contracts:
\begin{align}
    \mathcal{C}_{d}&=(true, \mathbf{OP}(r_1, r_2))\label{eq:cd}\\
    \mathcal{C}_{n}&=(true, \mathbf{OP}(r_3, r_4))\label{eq:cn}\\
    \mathcal{C}_{g}&=(\varphi^\text{fair}_{s}, \mathbf{BD}(person, greet))\label{eq:cg}\\
    \mathcal{C}_{r}&=(\varphi^\text{fair}_{s}, \mathbf{BR}(person, register))\label{eq:cr}
\end{align}
Where $\varphi^\text{fair}_{s}$ represents a \textit{fairness} assumption on the sensor variables, i.e. $\textbf{G}(\textbf{F}(person))$, since we expect to see a person infinitely often. 

\subsection{Checks}
\NAME check that a any contract is always \textit{compatible}, \textit{consistent}, and \textit{feasible}. Given a contract $\mathcal{C}=(\psi, \phi)$, we have that:

\begin{align}
    \mathcal{C} ~~\text{is compatible} & &\textbf{iff}~~~~& \psi ~~\text{is}~~ \textit{satisfiable}\\
    \mathcal{C} ~~\text{is consistent} & &\textbf{iff}~~~~& \phi ~~\text{is}~~ \textit{satisfiable}\\
    \mathcal{C} ~~\text{is feasible} & &\textbf{iff}~~~~& (\psi \land \phi) ~~\text{is}~~ \textit{satisfiable}
\end{align}

From now on we assume that every contract is compatible consistent and feasible and we say that the contract is \textit{well-formed.} \pierg{@pierl, can we use 'well-formed'? I don't see the use of it in Benveniste paper..} \pierl{Well, if a contract is feasible, then it is both compatible and consistent. I think we can use a property like well-formedness, but do we need it, if we coined `feasible'? `Feasible' is also not in the monograph.}

\subsubsection{Operations}
\NAME supports the operations of \textit{composition} and  \textit{conjunction} among contracts. Let $\mathcal{C}_1=(\psi_1, \phi_1)$ and $\mathcal{C}_2=(\psi_2, \phi_2)$ be two contracts.

The \textit{composition} $\mathcal{C}_1 ~||~ \mathcal{C}_2$ results in a contract $\mathcal{C}^{||} = (\psi^{||}, \phi^{||})$ such that:
\begin{align}
    \psi^{||} & = \psi_1 \land \psi_2 \lor \neg(\phi_1 \land \phi_2)\\
    \phi^{||} & = \phi_1 \land \phi_2
\end{align}

The \textit{conjunction} $\mathcal{C}_1 ~\land~ \mathcal{C}_2$ results in a contract $\mathcal{C}^{\land} = (\psi^{\land}, \phi^{\land})$ such that:
\begin{align}
    \psi^{\land} & = \psi_1 \lor \psi_2 \\
    \phi^{\land} & = \phi_1 \land \phi_2
\end{align}

\pierl{Double-check punctuation throughout the text.}

\subsubsection{Comparisons}
As with the specification, we can compare contracts. Let us consider the contracts $\mathcal{C}_1=(\psi_1, \phi_1)$ and $\mathcal{C}_2=(\psi_2, \phi_2)$; we have that:

\begin{align}
    \mathcal{C}_1 &== \mathcal{C}_2 &\textbf{iff}~~~~& (\psi_1 == \psi_2) & \land~~~~& (\phi_1 == \phi_2)\\
    \mathcal{C}_1 &\neq \mathcal{C}_2 &\textbf{iff}~~~~& (\psi_1 \neq \psi_2) & \lor~~~~& (\phi_1 \neq \phi_2)\\
    \mathcal{C}_1 &\leq \mathcal{C}_2 &\textbf{iff}~~~~& (\psi_1 \ge \psi_2) & \land~~~~& (\phi_1 \le \phi_2)\\
    \mathcal{C}_1 &\geq \mathcal{C}_2 &\textbf{iff}~~~~& (\psi_1 \le \psi_2) & \land~~~~& (\phi_1 \ge \phi_2)\\
    \mathcal{C}_1 &< \mathcal{C}_2 &\textbf{iff}~~~~& (\mathcal{C}_1 \leq \mathcal{C}_2) & \land~~~~& (\mathcal{C}_1 \neq \mathcal{C}_2)\\
    \mathcal{C}_1 &> \mathcal{C}_2 &\textbf{iff}~~~~& (\mathcal{C}_1 \geq \mathcal{C}_2) & \land~~~~& (\mathcal{C}_1 \neq \mathcal{C}_2)
\end{align}

\pierl{Not sure about these notations, and whether we need all of them.}

\subsection{\textbf{Goal}}

In \NAME, each mission requirement is modeled by a goal, which is characterized by the following elements:
\begin{itemize}
    \item \textit{Name}: goal identifier; 
    \item \textit{Description}: English description of the mission requirement;
    \item \textit{Context}: Specification containing a Boolean predicate expressed on types of kind 'context';
    \item \textit{Contract}: a Contract object formalizing the objective of the goal.
    \item \textit{Controller}: Mealy machine realizing the contract associated to the goal.
    \item \textit{World}: \textit{World} object where the goal will be deployed.
\end{itemize}

\textit{Contexts} are formalized in terms of Boolean predicates encoding the situation in which a goal must be active. For example, context propositions can encode information related to the location, time, or identities associated with a goal. In a robotic application, locations specify \emph{where} a robot can be, time specifies \emph{when} a particular goal must be active (e.g., during the day or the night), and identities specify the state of external entities (\emph{who}) that may interact with the robot.

\textit{Contracts} can be built up from specification using, for example, robotic patterns to indicate what is the objective of the robot in the goal being modeled. There is always only one contract associated with each goal. We will refer the contract belonging \pierl{?} to the goal $\mathcal{G}_i$ with $\mathcal{C}_i$. Also, we refer to any contract operation among goals to be related to the contracts forming the goals.

\textit{Controllers} are generated by realizing the specification associated with the contract \pierl{?}. Specifically, if the guarantees of the contract $\psi \rightarrow \phi$ is a specification realizable in a controller, then a finite state machine that satisfies the specification is produced, i.e., the \textit{controller}.

The \textit{world} object is needed to extract all the refinement, adjacency, and mutually exclusion rules that the robot is subject to in the mission. Such rules will add constraints on the robot behavior and jeopardize \pierl{?} the missions' satisfiability or realizability according to the world configuration.

\subsubsection{Checks, Comparisons, and Operations}
We reduce all the formal operations, checks, and comparisons among goals to their corresponding contracts.
Goal conflicts are detected by checking the contract's compatibility, consistency, and feasibility formalizing the goals. 
\NAME links the conflicting clauses in the contract specifications to the goals generated and presents them to the designer. 



==> Tex/introduction_orig.tex <==
\section{Introduction}

Robotic missions are increasingly being deployed across various fields, such as space exploration, healthcare, search and rescue, and industrial manufacturing. Nevertheless, the effective specification and implementation of these missions continue to be significant challenges in software engineering for robotics. We define \emph{mission requirements} as descriptions of the robotic mission in natural language, while \emph{mission specifications} are the formulation of these requirements in a logical language with precise semantics~\cite{SpecificationPatternsTSE}.

Recent years have seen various proposals for specifying missions, for instance, using logics~\cite{menghi2018multi,ulusoy2011optimal,fainekos2009temporal,guo2013revising,wolff2013automaton,kress2011robot,doi:10.1177/0278364914546174,DBLP:journals/corr/MaozR16,maoz2011aspectltl,maozsynthesis,MaozFSE}, state charts~\cite{bohren2010smach,thomas2013new,klotzbucher2012coordinating}, Petri nets~\cite{wang1991petri,ziparo2008petri}, domain-specific languages~\cite{GLRSWWCA12,campusano.ea:2017:live,DBLP:journals/corr/SchwartzNAM14,Ruscio2016,Bozhinoski2015,Ciccozzi4496,Doherty2012}, or robotic patterns~\cite{SpecificationPatternsTSE,TSE2023}. However, the task of writing mission specifications that accurately reflect the mission requirements remains challenging and cumbersome. This difficulty is amplified by the variability of conditions and application scenarios that the system may encounter in real-world operational environments. Furthermore, the increased complexity of mission specifications can render the generation of a correct-by-construction implementation, such as through synthesis methods, intractable. 

Addressing the complexity of mission specifications by breaking them down into smaller, more manageable pieces is one approach. However, large and complex specifications can be difficult to comprehend and manage, posing challenges to their decomposition into component parts. Consequently, frameworks that can effectively guide the implementation of robotic mission specifications in a modular way, through the composition of sub-missions while guaranteeing correctness, are highly sought after.

In this paper, we propose a framework for the specification and implementation of contextual robotic missions, utilizing assume-guarantee contracts to structure a complex mission in a hierarchical and modular fashion as an 
aggregation of smaller sub-missions, which we term \emph{tasks}. 
We introduce the Contract-based Goal Graph (CGG) as a key element of our framework. The CGG is a formal model used to organize and represent the mission's objectives hierarchically. It serves as an analytic tool to delineate and correlate the relationships between tasks.
Each task is associated with a specific \textit{context}~\cite{mallozzi2020crome}, defined as a set of environmental conditions (environment states) that may occur during a mission. We define a \textit{mission scenario} as a collection of tasks with compatible contexts. All mission scenarios are linked to contexts that are mutually exclusive, ensuring that at any given time, only one context and one scenario are active. Furthermore, each scenario can be realized into a controller, which is a finite state machine that dictates the robot's behavior in response to environmental inputs. 
In this work, we focus on reactive synthesis from Linear Temporal Logic (LTL), a robust methodology for specifying and validating the behavior of reactive systems like robots in dynamic environments.
To fulfill a contextual mission, the robot must transition between mission scenarios as the context shifts, leading to a \textit{context switch}. We propose a method to dynamically alternate between task controllers while assuring the correctness of the entire mission.

Some results of this paper were initially presented in our conference submission, which introduced 
\NAME~\cite{mallozzi2020crome}, 
employing contracts~\cite{benveniste2018contracts,Nuzzo15b} and context to formalize mission tasks, along with robotic patterns to translate mission requirements into specifications. In the current paper, we enhance \NAME by introducing two significant advancements. First, we unveil an improved version of the formal model, the \textit{Contract-based Goal Graph} (CGG), which offers a structured graphical representation of the mission specification. Second, we develop a methodology for dynamically generating a plan that continuously satisfies the mission specification, even amidst context changes. This is accomplished by associating controllers with each mission scenario, facilitating efficient synthesis and providing a mechanism for automatic transitioning between controllers while upholding the mission's overall objectives.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{figures/illustrative-example-DYNACROME}
  \caption{Running example map consisting of five regions and two contexts.}
  \label{fig:illustrative}
\end{figure}

\subsection{Running Example} \label{sec:running}

We model time as an infinite sequence of discrete intervals. At each interval, the robot can be located in one of the five regions depicted in the map in Figure~\ref{fig:illustrative}, denoted by \( r_1, r_2, r_3, r_4, r_5 \), and can transition from one region to an adjacent one within a single time step. We assume two mutually exclusive contexts: \textit{day} and \textit{night}. A single sensor is employed to detect the presence of a person, denoted by \textit{person}, and two actions are available: \textit{greet} and \textit{register}.

The mission's objective is to continuously navigate different regions in a manner contingent on the context. During the day, the robot is required to sequentially visit regions \( r_1 \) and \( r_2 \), commencing from \( r_1 \). At night, it should visit regions \( r_3 \) and \( r_4 \) in order, starting from \( r_3 \). Upon a change in context, the robot must resume the sequence of visits from the last region it was in. To transition between regions \( r_1, r_2 \) and \( r_3, r_4 \), the robot must traverse region \( r_5 \), necessitating an additional time step. Additionally, when the robot detects a person in any region, it promptly performs the greeting action. During the day, if a person is detected, the robot is also expected to register them in the following step. Our aim is to devise a controller capable of managing any context switch and fulfilling the mission requirements.

\subsection{Motivation}

Expressing a mission specification, such as the one in Section~\ref{sec:running}, in a formal language such as linear temporal logic (LTL)~\cite{pnueli1977temporal} can be challenging, due to 
\textit{1) the need to effectively capture different  contexts} and \textit{2) the need to track the current status every time the context switches}.

Accurately modeling the behavior of the context variables is key to the satisfaction of contextual missions. In fact, leaving them unconstrained could allow for behaviors in which the context switches infinitely often or not at all, forcing the robot to fail to achieve the mission. This is the case, for instance, in our running example, if the context variable switches at every step from \textit{day} to \textit{night}, since 
\textit{passing through} region $r_5$ at any context switch would require an extra time step. On the other hand, constraining the  behavior of the context variables, e.g., by specifying minimum or maximum duration intervals, may be impractical in LTL. Furthermore, associating a task to a context may require \emph{ad hoc} manipulation of the logic formula encoding the task, which may vary based on the specific task. 
For example, prescribing that the task LTL formulas $\varphi_1=\mathsf{G}(p_1 \rightarrow p_2)$ and $\varphi_2=(p_1 ~\mathsf{U} ~p_2)$ must hold under context $x$, where $p_1$, $p_2$, and $x$ are atomic propositions, would require rewriting the formulas as 
$\varphi_1'=\mathsf{G}((p_1 \land x) \rightarrow (p_2 \land x))$ and 
$\varphi_2'=(((p_1 \land x) \lor \overline{x}) ~\mathsf{U} ~(p_2 \land x))$ to embed the context.

Finally, the robot must remember the last visited state when the context switches. In our example, if the context switches while the robot is in $r_1$, the next time the context transitions to \textit{day} again, the robot must start from the state \textit{after} $r_1$, i.e., $r_2$. Tracking the current state would require extra  variables and impractical modification of the LTL task formulas to account for the state of these variables.

\subsection{Paper Roadmap}
The rest of the paper is organized as follows. In Section~\ref{sec:background}, we provide a background on assume-guarantee contracts, linear temporal logic, and reactive synthesis. In Section~\ref{sec:problem}, we define the problem of satisfying a contextual mission. In Section~\ref{sec:cgg}, we introduce the \textit{Contract-Based Goal Model} (CGG), which is the formal model developed by \NAME to represent contextual missions. In Section~\ref{sec:orchestration}, we present how \NAME produces robotic plans that consistently satisfy the mission under changing contexts. In Section~\ref{sec:implementation} and Section~\ref{sec:evaluation}, we provide details on the implementation of \NAME and evaluate our approach. Finally, in Section~\ref{sec:related}, we discuss related works in various areas, and we conclude in Section~\ref{sec:conclusion}.

==> Tex/orchestration_orig.tex <==

\section{Controller Orchestration}
\label{sec:orchestration}

\NAME ensures seamless switching between task controllers to satisfy the contextual mission by leveraging a combination of task and transition controllers. Task controllers are synthesized from the specifications of each mission scenario. Transition controllers guide the robot from one task controller to another when a context switch occurs.

Each controller is a Mealy machine evolving in a subset of the robot's state, input, and output space. The challenge is to orchestrate all the controllers, while ensuring that the robot always satisfies the contextual mission.

\subsection{Task and Transition Controllers}

\begin{figure*}[]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/example-active-controllers.eps}
    \caption{A specification and transition controller that have been modified with the activation inputs.} 
    \label{fig:active-controllers}
\end{figure*}
  
  We use a set of task controllers to realize the mission scenario in each context.

  \begin{definition}[Task Controllers]
  Given a contextual mission specification $\Gamma=(\gamma_1, \gamma_2, \ldots, \gamma_n)$, we define the set of \textit{task controllers} $\Lambda = (\lambda_1, \lambda_2, \ldots, \lambda_n )$ where, for all $1 \leq i \leq n$, controller $\lambda_i\in \Lambda$ realizes specification $\gamma_i \in \Gamma$.
  \end{definition}
  
  We then resort to additional controllers to guide a robot's transition between mission scenarios.
  
  \begin{definition}[Transition Controllers]
  We define a \textit{transition controller} $k_{r_i, r_j}$ \pierl{why task controllers use greek letters while this is not the case for transition controllers?} as a state machine \pierl{?} that transitions from region $r_i$ to region $r_j$, in the least number of steps, where $r_i$ and $r_j \in R$ and $i \neq j$. We define $K$ to be the set of all possible transition controllers, including a controller for each pair of regions $r_i, r_j \in R$. That is, $K = \{k_{r_ir_j}: r_i,r_j \in R, i \neq j \}$.
  \end{definition}
  
  In our example, when the context switches from day to night, the robot must switch from patrolling regions $r_1$ and $r_2$ to patrolling regions $r_3$ and $r_4$. Immediately after a context switch there is a \textit{transition phase} in which the robot is guided by a controller from a region in $\{r_1, r_2\}$ to a region in $\{r_3, r_4\}$. A context switch can happen while the robot is operating in any of the four regions above. 
  
  \begin{definition}[Transition Time]
  We define the \textit{transition time} $t_{\texttt{trans}}$ to be the maximum among the numbers of time steps needed for any controller $k_{r_i, r_j} \in K$ to transition from $r_i$ to $r_j$.
  \end{definition}
  
  The orchestration system \pierl{Have we ever defined this system? Is that a centralized controller? Or just the design methodology?} coordinates the task and transition controllers so that the robot satisfies the contextual mission, as further detailed below. 
  
\subsubsection{\textbf{Active Controllers}}

\NAME introduces the notion of \textit{active} and \textit{inactive} controllers to modify task and transition controllers and facilitate their coordination. Controllers are finite state machines, specifically Mealy machines.  
Two new sets of atomic propositions are defined:
\begin{align*}
    \mathcal{I}_\Lambda^\textbf{a}&=\{\textbf{a}_1, \textbf{a}_2,...,\textbf{a}_n\}\\
    \mathcal{I}_K^\textbf{a} &=\{\textbf{a}_{r_ir_j}: r_i,r_j \in R, i \neq j\}
\end{align*}
These sets of propositions are used as additional inputs for the controllers and are referred to as \textit{activation inputs}.

For a task controller $\lambda_i \in \Lambda$, an atomic proposition $\textbf{a}_i \in \mathcal{I}_\Lambda^\textbf{a}$ is added to its inputs. \pierl{notation?} A self-loop transition is added to any state of $\lambda_i$, which accepts the negation of $\textbf{a}_i$ as input and leaves the output undetermined (\textendash). \pierl{Ever defined?}
For any transition controller $k_{r_ir_j} \in K$, an atomic proposition $\textbf{a}_{r_ir_j}$ is added to its inputs. Two loop transitions are further added, one to its initial state and one from its terminal state to its start state. \pierl{?} Both loop transitions accept the negation of $\textbf{a}_{r_ir_j}$ as input for any other input of $k_{r_ir_j}$ and leave the output to be undetermined (\textendash). 
The modified task and transition controller sets are denoted by $\Lambda'=\{\lambda_1', \lambda_2',...,\lambda_n'\}$ and $K'=\{k'_{r_ir_j}: r_i,r_j \in R, i \neq j\}$, respectively.

A controller $\lambda_i' \in \Lambda'$ or $k'_{r_ir_j} \in K'$ is considered \textit{active} if its activation input is set to \textit{true}, and \textit{inactive} otherwise. Figure~\ref{fig:active-controllers} illustrates two modified controllers. The task controller $\Lambda_1$ has inputs $\textbf{a}_1$, $p$, outputs $r_1$, $r_2$, $g$, start state $0$, and no terminal state. The transition controller $k_{r_1r_3}$ has inputs $\textbf{a}_{r_1r_3}$, $p$, outputs $r_1$, $r_3$, $r_5$, $g$, start state $0$, and terminal state $3$. \NAME adds the \textit{activation inputs} $\textbf{a}_1$ and $\textbf{a}_{r_1r_3}$ and the transitions represented by dashed lines in Figure~\ref{fig:active-controllers}. These two controllers are generated from the specification resulting from the composition of goals $\mathcal{G}_d$ and $\mathcal{G}_g$, i.e., patrol during the day and greet immediately when a person is detected. \pierl{why composition?}

The traces produced by $\lambda_i' \in \Lambda'$ are equivalent to the traces produced by $\lambda_i \in \Lambda$ when $\lambda_i'$ is \textit{active}. \pierl{What does it mean for traces to be equivalent? Ever defined?} Similarly, the traces produced by $k_{r_ir_j}' \in K'$ are equivalent to the ones produced by $k_{r_ir_j} \in K$ when $k_{r_ir_j}'$ is \textit{active}. If the activation inputs of $\Lambda'$ and $K'$ are always \textit{true}, then their behaviors are equivalent to those of $\Lambda$ and $K$.

\subsubsection{\textbf{Composition}}
Given a set of controllers $\Lambda^*= \Lambda' \cup K'$ where each element $\lambda^i \in \Lambda^*$ \pierl{now we have the index as exponent?} is a finite state machine $\lambda^i=(S^i, \mathcal{I}^i, \mathcal{O}^i, s_0^i, \delta^i)$, $N = |\Lambda^*|$, and  where $\textit{in}^i_t$ and $\textit{out}^i_t$ are respectively the inputs and outputs of $\lambda^i$ at time $t$. We indicate with subscripts $s^i_0$, $s^i_t$ and $s^i_{t+1}$ the state of $\lambda^i$ at time $0$, $t$ and $t+1$, respectively. We define the composition of all the elements in $\Lambda^*$ as a finite-state machine $\Lambda^{||}=(S^{||}, \mathcal{I}^{||}, \mathcal{O}^{||}, s_0^{||}, \delta^{||})$ where:
\begin{align*}
    S^{||} &= S^1 \times S^2 \times ... \times S^N\\
    \mathcal{I}^{||} &= \mathcal{I}^1 \times \mathcal{I}^2 \times ... \times \mathcal{I}^N\\
    \mathcal{O}^{||} &= \mathcal{O}^1 \times \mathcal{O}^2 \times ... \times \mathcal{O}^N\\
    s^{||}_0 &= (s_0^1, s_0^2,...,s_0^N)\\
    \delta^{||} &:S^{||} \times \mathcal{I}^{||} \rightarrow S^{||} \times \mathcal{O}^{||}
\end{align*}

At each step, the transition function $\delta^{||}$ produces a new state and output as follows:
\begin{align*}
    &~((s^1_{t+1}, s^2_{t+1}, ..., s^N_{t+1}), (\textit{out}^1_{t}, \textit{out}^2_{t}, ..., \textit{out}^N_{t})) \\
    =&~\delta^{||}((s^1_{t}, s^2_{t}, ..., s^N_{t}), (\textit{in}^1_{t}, \textit{in}^2_{t}, ..., \textit{in}^N_{t}))
\end{align*}
where $(s^i_{t+1}, \textit{out}^i_{t}) = \delta^i(s^i_{t+1}, \textit{in}^i_{t})$ for $i=\{1, \ldots, N\}$. \pierl{Is the composition the classical one, as defined by the synchronous reactive model of computation? I don't think we need $t$, etc. State machines have no time.}
The composition is well-defined, i.e., there are no conflicting outputs, 
by construction, since each Mealy machine relates to a different mission scenario, and there is only one active scenario at each time.

\subsection{The Orchestration System}

The orchestration system is responsible for monitoring the active context $x_i \in X$ and coordinating the behavior of the finite state machine $\Lambda^{||}$ to ensure that it fulfills the mission. To achieve this, the orchestration system controls the activation inputs of $\mathcal{O}^{||}$, which determines its outputs. If any output $o_t \in \mathcal{O}^{||}$ is not determined by any machine $\lambda_i \in \Lambda*$ at time $t \in \mathbb{N}$, then it assigns $o_t = \textit{false}$.

We represent the orchestration system as a network of timed automata. Timed automata are finite state machines extended with clock variables. In our case, we use 
discrete-time ticks. Each system involved in the orchestration \pierl{what does it mean?} is represented as a template automaton. Figure~\ref{fig:automata} shows the templates for the different systems involved in the orchestration. Transitions can be labeled with synchronization channels, guards, or updates. \pierl{defined?} State invariants, indicated in Figure~\ref{fig:automata} next to states, are conditions that must be satisfied while the automaton is in that state. Updates can be simple assignments or entire functions, and we use the notation $name:=value$ to indicate an assignment, distinguishing it from a predicate ($name = value$).

\begin{figure}[]
  \centering
  \includegraphics[width=1\linewidth]{figures/automata.eps}
  \caption{Timed automata that model the interactions among the orchestrator, contexts and controllers.
  Gray states represents \textit{committed} locations. \pierl{???}} 
  \label{fig:automata}
\end{figure}

\subsubsection{Template Instances}

There are $n$ instances of the \textit{Context} template, each modeling a different context. In addition, we have $(n^2 - n)$ instances of the $\textit{T-Automaton}$ template, each modeling a \textit{transition controller} from context $x_i$ to context $x_j$ where $i \neq j$. For each \textit{task controller}, we have an associated instance of the $\textit{S-Controller}$ template. There is one $\textit{S-Controller}$ instance for each \textit{Context} instance. Finally, the $\textit{Orchestrator}$ automaton coordinates the states of all the instances of the \textit{Context}, $\textit{S-Controller}$, and $\textit{T-Automaton}$ templates. In the following, we will refer to contexts, task automata, and transition automata to indicate the instances of the corresponding templates. We will use the abbreviated notation $C[i]$, $S[i]$, and $T[i][j]$ to indicate specific instances of contexts, specification and transition automata, respectively. Finally, we will use $O$ to indicate the orchestration automaton.

\subsubsection{Synchronization Channels}

The coordination among automata happens via the synchronization of the transitions of different automata on binary synchronization channels. An edge labeled with $channel!$ synchronizes with another labeled $channel?$. Given $n$ contexts, we have defined the following synchronization channels:

\begin{itemize}
\item $n$ $active$ channels, one channel for each context, where each channel gets fired when a context becomes active. \pierl{firing a channel?}
\item $n$ $go$ and $n$ $stop$ channels, to activate and deactivate, respectively, the task automata.
\item $(n^2 - n)$ $transit$ and $(n^2 - n)$ $done$ channels, respectively, to activate each transition automaton and to get notified when it has terminated its execution.
\item $cs$ is one \textit{broadcast channel} where one sender ($cs!$) can synchronize with an arbitrary number of receivers ($cs?$). It is used to notify all contexts of a context switch.
\end{itemize}

\subsubsection{States}
\emph{Committed locations} (represented in gray in Figure~\ref{fig:automata}) are states where time delay is not allowed, and the only possible transition is the one outgoing from the committed location. Thus, all actions from/to a committed state are considered atomic.

Initially, all automata are in the \textit{idle} state. At any other given moment, context, transition, and task automata can either be in the \textit{active} or the \textit{idle} states, while the orchestrator can be in the \textit{spec} or \textit{transit} states.

\subsubsection{Local Clock Variables}
Contexts and transition automata have a local clock variable, i.e., $t^x$ and $t^t$ respectively. The contexts use $t^x$ to measure the \textit{minimum} time they are required to be active. The transition automata use $t^t$ to bound the \textit{maximum} time they can be active. Both clock variables are reset every time the automata move to their \textit{active} states.

\subsubsection{Synchronization with Mealy Machines}

Timed automata model the \textit{dynamic behavior} of the system and have a precise notion of \textit{time}~\cite{behrmann2006uppaal}, while the Mealy machine determines what the robot should do when it reacts. However, there are no constraints on \textit{when} the reaction should happen.

The timed automata modeled in Uppaal \pierl{The tool does not matter at this stage. Let us separate the models from their implementations} use a \textit{continuous time model} \pierl{I believe we are using discrete models?}. We have local clocks to every state machine that determine when a transition should fire and synchronize with another transition if a synchronization channel is present \pierl{this is confusing, since we said that Mealy state machines do not have clocks.}. Let us define when the Mealy machine reactions happen and how they synchronize with the timed automata.

We discretize time into fixed time units $t$. At each $t$, a transition can be taken by any timed automata (e.g., if the transition guards allow it). In parallel with the timed automata, at each $t$, a reaction must happen in every Mealy machine participating in the composition $\Lambda^{||}$. That is, at every $t$, each Mealy machine evaluates its inputs and sets its outputs. Most of the Mealy machines in $\Lambda^{||}$ will not be active. In fact, only one transition controller or one task controller will be active. The activation of the controllers is set by the timed automata as follows.

The \textit{\textbf{trans\_start()}}, \textit{\textbf{trans\_end()}}, \textit{\textbf{activate()}}, and \textit{\textbf{deactivate()}} functions are executed every time a transition is taken from \textit{idle} to \textit{active} in a transition or task automaton. These functions are responsible for managing the activation inputs in $\mathcal{I}^{||}$ and, consequently, affecting the behavior of $\Lambda^{||}$.
Specifically, for any task automaton $S[i]$ and transition automaton $T[i][j]$:

\begin{itemize}
\item $activate()$ sets to true the activation input of the Mealy machine $\lambda_i'$, which is the only machine related to the task automaton $S[i]$. It also sets the output $Active \in \mathcal{O}$ to true.
\item $deactivate()$ sets to false the activation input of the Mealy machine $\lambda_i'$. It also sets $Active$ to false.
\item $trans\_start()$ sets to true the activation input of a Mealy machine $k'_{r_ir_j} \in K'$, where which Mealy machine to activate depends on the current region of the robot $r_i$ and its destination $r_j$.
\item $trans\_end()$ sets to true the activation input of $k'_{r_ir_j} \in K'$ to false \pierl{unclear}.
\end{itemize}

\begin{remark}
\label{rem:active}
$Active \in \mathcal{O}$ is \textit{true} if and only if any task automaton is in the \textit{active} state.
\end{remark}

\subsection{Proof of Correctness}
We prove that our system produces traces that always satisfy the contextual mission as defined in Section~\ref{sec:problem}. We construct the proof incrementally, starting by proving the following properties of the orchestration system:

\begin{itemize}
\item Initially, all automata are in the \textit{idle} state and wait for a context to become active.
\item After the first context becomes active, there is exactly one context active at all times.
\item Any context stays active for at least $t_{\texttt{context}}$ time units.
\item No context can become active for two consecutive time units.
\item After the first context has become active, there is always one task automaton or one transition automaton active, but they are never active together.
\item Transition automata can be active at most $t_{\texttt{trans}}$ time units.
\item Every time a context becomes active after at most $t_{\texttt{trans}}$ time units, the task automaton related to the active context also becomes active.
\end{itemize}

In the following, we assume that all the automata start
in the \textit{idle} state.

\begin{lemma}
\label{lem:contextfirst}
Under the initial condition, no automaton can take a transition except for a context, and precisely one context can transition to the \textit{active} state.
\end{lemma}

\begin{proof}
We will prove this by induction on the number of contexts.

\vspace{2mm}
\noindent\textbf{Base case $n=1$:} In this case, we only have one context $C[0]$, one orchestrator $O$, and one task automaton $S[0]$. $O$ and $S[0]$ are waiting on the synchronization channels $active$ and $go$, respectively. $cs_enabled$ is initially set to $true$, so $C[0]$ is free to move from \textit{idle} to \textit{active}. The atomic transition from idle to active is synchronized on the $cs$ and $active$ channels. It first sends on the broadcast channel $cs!$, which is non-blocking and has no effect since no other context is enabled to receive on $cs?$. In the same transition, it synchronizes with the orchestrator via the $active[0]$ channel, and the orchestrator can now synchronize with $S[0]$ via the $go[x]$ channel. Thus, initially, no other automaton can move from the \textit{idle} state but the context automaton $C[0]$.

\vspace{2mm}
\noindent\textbf{Induction hypothesis:} Let us assume that our lemma holds for a number of contexts $n=k$.

\vspace{2mm}
\noindent\textbf{Induction step:} We will prove that the lemma holds for $n=k+1$. By adding an additional context, all contexts $C[0], C[1],...,C[k]$ are enabled to transition from the \textit{idle} to the \textit{active} state. By our induction hypothesis, we have that only one context, let's say context $C[i]$ ($0\leq i \leq k$), can effectively take the transition from \textit{idle} to \textit{active}, and by the base case (with $n=1$), as soon as $C[i]$ takes such transition, then $C[k+1]$ cannot do it. Thus, precisely one context can transition to the \textit{active} state, and no other automaton can take a transition under the initial condition.
We conclude the proof of Lemma~\ref{lem:contextfirst}.
\end{proof}

\pierl{Maybe this proof can be simplified. Not sure that we need induction here.}

\vspace{2mm}
\begin{lemma}
\label{lem:tcontext}
For any number $n$ of contexts, there is exactly one context in the \textit{active} state at any moment in time after the first context has become active. Any context stays in the \textit{active} state for at least $t_\texttt{context}$ time units.
\end{lemma}
\begin{proof}
According to Lemma~\ref{lem:contextfirst} contexts are the first automata to move. Initially, any instance can take the outgoing transition from the \textit{idle} state. Non-deterministically, one of the instances will set $cs\_enabled$ to false, and due to the atomicity guaranteed by committed states, all the other context instances will remain in the \textit{idle} state. The first context instance to take the transition sets $cs\_enabled$ to false before reaching the \textit{active} state so that no other context can become active. After $t_{\texttt{context}}$ time units the active context sets $cs\_enabled$ to true so that another context is enabled to become active.
As soon as another context exits from the \textit{idle} state, it synchronizes with the currently active context on the $cs$ channel so that the active context transitions to the \textit{idle} state. 
\end{proof}

\vspace{2mm}
\begin{lemma}
\label{lem:contextswitch}
No context can be activated twice in a row.
\end{lemma}

\begin{proof}
If a context $C[i]$ has already been activated, the only way for it to transition to the \textit{idle} state is by synchronizing on the $cs?$ channel. However, this can only happen when another context $C[j]$ becomes active, where $i \neq j$. Therefore, context $C[i]$ must wait for at least one other context to become active before it can be activated again.
\end{proof}

The orchestrator keeps track of the currently active context using a variable $cur$. When a new context instance $x$ becomes active, the orchestrator does the following:

\begin{enumerate}
\item It stops the execution of the currently active task automaton, i.e. $S[cur]$.
\item It activates the transition automaton from context $cur$ to context $x$, i.e. $T[cur][x]$.
\item It waits for the transition automaton to terminate its execution by waiting for the $done[cur][x]$ synchronization channel to fire.
\item It activates the task automaton of context $x$, i.e. $S[x]$.
\end{enumerate}

\begin{lemma}
    \label{lem:transspecmutex}
    After the first context becomes active, there is always either a task automaton or a transition automaton in the \textit{active} state, but never both at the same time.
    \end{lemma}
    \begin{proof}
    Operations 1), 2), and 4) are modeled as \textit{committed locations} in Figure~\ref{fig:automata} and are performed atomically by the orchestrator. The first time a context becomes active, the orchestrator activates a task automaton simultaneously with the context, ensuring that at least one automaton is in the \textit{active} state. During a context switch, the orchestrator stops the current task automaton, causing it to transition to the \textit{idle} state, and activates a transition automaton, which transitions to the \textit{active} state. At the same time instance, either the task automaton or the transition automaton is in the \textit{active} state, but never both. When the transition automaton terminates and transitions to the \textit{idle} state, it synchronizes with the orchestrator, which then activates the next task automaton in the same atomic operation, ensuring that there is always at least one automaton in the \textit{active} state.
    \end{proof}

\vspace{2mm}

\begin{lemma}
    \label{lem:ttrans}
    A transition automaton can be active for at most $t_{\texttt{trans}}$ time units.
    \end{lemma}
    \begin{proof}
    Due to the invariant in the \textit{active} state of the transition automaton, the automata must transition to the \textit{idle} state when $t^{t} \leq t_{\texttt{trans}}$.
    \end{proof}
    
\pierl{Do we mean larger than?}

\begin{theorem}
\label{thm:orchestration}
Given $n$ contexts, $n$ task automata, $n^2-n$ transition automata, and assuming $t_{\texttt{trans}} < t_{\texttt{context}}$, we have that:
\begin{itemize}
\item Every time a context $C[i]$ is active, then $S[i]$ becomes active after at most $t_{\texttt{trans}}$ time units and no transition or task automaton besides $S[i]$ can become active.
\end{itemize}
\end{theorem}

\begin{proof}
\emph{Initial phase:} If the orchestrator and automata are all in the \textit{idle} state, according to Lemma~\ref{lem:contextfirst} and Lemma~\ref{lem:transspecmutex}, the system is in the initial step waiting for one (and only one) context to become active. If $C[i]$ becomes active, then the orchestrator immediately activates $S[i]$ by synchronizing on the $go$ channel.

\emph{Context Switch:} Assume that we are in a condition where a context $C[j]$ is currently active (where $j \neq i$), then according to Lemma~\ref{lem:tcontext}, $C[i]$ cannot become active before $t_\texttt{context}$ time units. Assume that $C[i]$ becomes active $t_\texttt{context}$ time units after $C[j]$ became active, then according to Lemma~\ref{lem:ttrans}, and Lemma~\ref{lem:transspecmutex}, and our assumption that $t_{\texttt{trans}} < t_{\texttt{context}}$, we have that $S[j]$ must be active when $C[i]$ becomes active. The orchestrator will then stop $S[j]$ and activate $T[j][i]$. After at most $t_{\texttt{trans}}$ time units, $S[i]$ will become active. Because we assumed that $t_{\texttt{trans}} < t_{\texttt{context}}$ and we proved that 1) another context $C[j] \neq C[i]$ cannot become active before $t_{\texttt{context}}$ time units (Lemma~\ref{lem:tcontext}) and that 2) $C[i]$ cannot become active twice in a row (Lemma~\ref{lem:contextswitch}), we conclude that $S[i]$ must become active.
\end{proof}

\subsubsection{Starvation}
Our orchestration system assumes mutual exclusion between contexts and that they stay active for at least $t_{\texttt{context}}$ time units. However, we have no assumptions about how the contexts are scheduled. It is possible that some contexts may never become active, and as a result, the corresponding task automata will never be activated by the orchestrator.

\begin{remark}
Assuming a fair scheduler that activates all contexts infinitely often and that $t_{\texttt{trans}} < t_{\texttt{context}}$, we can conclude from Theorem \ref{thm:orchestration} that all task automata will be activated infinitely often, and no context (specification controller) will starve.
\end{remark}

\subsubsection{Model checking} We used UPPAAL\footnote{UPPAAL model available: \url{rebrand.ly/cromeuppaalmodel}}\cite{behrmann2006uppaal} to model the orchestration system as a network of timed automata shown in Figure\ref{fig:automata}. The automata are parametrized based on the number of contexts $N$. We successfully verified the model against the following properties:

\begin{center}
\textit{`There is never more than one T-Automaton active at any given time'}\\

    \texttt{A[] forall (i: N) forall (j: N) forall (l: N) forall (m: N) T\_automaton(i,l).Active \& T\_automaton(j,m).Active imply (i==j \& l==m)}
\end{center}

\begin{center}
\textit{`There is always at most one context active at any given time'}\\

    \texttt{A[] forall (i: N) forall (j: N) Context(i).Active \& Context(j).Active imply (i==j)}
\end{center}

\begin{center}
\textit{`There is always at most one S-automaton active at any given time'}\\

    \texttt{A[] forall (i: N) forall (j: N) S-automaton(i).Active \& S-automaton(j).Active imply (i==j)}
\end{center}

\begin{center}
\textit{`If any context becomes active its S-automaton will eventually become active'}\\
    \texttt{Context(i).Active --> S\_automaton(i).Active}
\end{center}

\begin{center}
\textit{`There are no deadlocks'}\\
    \texttt{A[] not deadlock}
\end{center}

\begin{theorem}
    \label{thm:missionsatisfaction}[Mission Satisfaction]
    Given a contextual mission $\mathcal{M} = (X, \Gamma, AC, CT)$, and assuming that:
    \begin{enumerate}
    \item for every specification in $\gamma$ there is a task controller $\lambda$ that realizes it;
    \item there is a transition controller $k$ for every possible context switch and where $t_{\texttt{trans}} < t_{\texttt{context}}$.
    \end{enumerate}
    
    Then the behaviors produced by $\Lambda^{||}$ together with the orchestration system of \CROME will always satisfy the contextual mission as defined in Section~\ref{sec:problem}.
    \end{theorem}
    
    \begin{proof}
    Theorem~\ref{thm:orchestration} guarantees that for any context becoming active, the orchestration system guarantees that a task automaton will become active after at most $t_\texttt{trans}$ time units. The behavior of the task and transition automata is linked to the \textit{actual} (i.e., the Mealy machines) task and transition controllers via the execution of the \emph{activate()}, \emph{deactivate()}, \emph{trans\_start()} and \emph{trans\_end()} functions. When the functions are not fired, the Mealy machines react synchronously with the ticks of the timed automata.
    
    Let $x_i \in X$ become active at time $t \in \mathbb{N}$ where $CT(ACT(t)) = \gamma_i$ and $\lambda_i \models \gamma_i$. The behavior produced by $\lambda_i'$ is equivalent to $\lambda_i$ when $\lambda_i'$ is active. According to the remark in Section~\ref{rem:active}, \textit{Active} is true if and only if a task automaton is in the active state.
    
    Since $\lambda_i$ satisfies $\gamma_i$ by construction, we have that the mission $\mathcal{M}$ is always satisfied by the robot $\mathcal{R}$ according to the definition of satisfaction defined in Problem 2 of Section~\ref{sec:problem}. Therefore, for any context $x_i$ becoming active, the behavior produced by $\Lambda^{||}$ together with the orchestration system of \CROME will always satisfy the contextual mission. Since the theorem holds for any $x_i \in X$, it holds for all $x \in X$, and the theorem is proved.
    \end{proof}



==> Tex/problem-definition_orig.tex <==

\section{Problem Definition}
\label{sec:problem}

Robotic missions specify what the robot should accomplish under different environmental conditions or \textit{contexts}. We model each robot objective in terms of \textit{goals} and formalize each goal in terms of \textit{contracts}. We provide an overview of the fundamental building blocks of our framework and demonstrate how they contribute to producing robot behaviors that satisfy the mission. We assume that time is discrete, and we refer to a finite sequence of steps as a \textit{time interval} or \textit{time frame}.

We represent the mission specification as sets of behaviors.

\begin{definition}[Behavior]
A \textit{behavior} is an assignment of values to all system (robot and environment) variables for all natural numbers. We refer to the value of a variable at natural number $i$ as the value of that variable at \emph{step} $i$.
\end{definition}

\begin{definition}[Mission Contexts]
    Let $X={x_0, x_1, \dots, x_n}$ be the set of \textit{mission contexts}. Each $x_i \in X$ represents a Boolean condition that is evaluated over the natural numbers, such that $x_i: \mathbb{N} \rightarrow \{\textit{true}, \textit{false}\}$.
    \end{definition}
    
    \noindent \textbf{Assumptions:}
    \begin{itemize}
    \item The contexts in $X$ are mutually exclusive. That is, for every $x_i, x_j \in X$ (with $i \neq j$), if $x_i$ is \textit{true} at any given time-step, then $x_j$ must be \textit{false}.
    \item Every context $x_i \in X$ is \textit{true} infinitely often, i.e., $\textsf{G}(\textsf{F}(x_i))$ holds for all $x_i \in X$.
    \item Every context is \textit{true} for at least $t_{\texttt{context}}$ consecutive time steps.
    \end{itemize}
    
    A context represents a Boolean condition that reflects the robot's environment, such as whether it's raining or not, or whether it's day or night. Contexts are used to state requirements under varying conditions in the environment. At any given time-step during the mission, at most one context is \textbf{active}, i.e., the context that is currently \textit{true}. Multiple contexts can be active during the mission, but not simultaneously. A \textbf{context switch} is an uncontrollable event that can happen at any point in time during the execution of the mission. When a context switch occurs, the current active context becomes inactive, and a different context becomes active. Both events occur instantaneously in the same time step. We have added a simple fairness assumption as we do not put a bound on how many times every context can become active.
 
We model the robot as set of behaviours over the sets of atomic propositions $\mathcal{I}$ and $\mathcal{O}$ representing the inputs and outputs of the robot respectively.

\begin{definition}[Robot Behavior]
A robot behavior $w$ is an assignment to $\mathcal{I}$ and $\mathcal{O}$ for all time steps. That is, a behavior is $w = (w_0^{\mathcal{I}}, w_0^{\mathcal{O}}),(w_1^{\mathcal{I}}, w_1^{\mathcal{O}}),(w_2^{\mathcal{I}}, w_2^{\mathcal{O}}), \ldots \in (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega$. We indicate with $w_t = (w_t^{\mathcal{I}}, w_t^{\mathcal{O}})$ the input and output values at time $t$. 
\end{definition}

\begin{definition}[Projected Robot Behavior]
    Given a function $R: 2^{\mathbb{N}} \times (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega \rightarrow (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega$ that takes in input a set $H$ of natural numbers and a robot behaviour $w$, the \textit{projected robot behaviour} $R(H, w)$ is the trace $(w^{\mathcal{I}}_{t_0}, w^{\mathcal{O}}_{t_0}),(w^{\mathcal{I}}_{t_1}, w^{\mathcal{O}}_{t_1}),  \ldots $, where $t_0$ is the smallest element of $H$, $t_1$ the next smallest element, and so on.
\end{definition}

The projected robot behavior is obtained by restricting the input behavior to the set of time steps specified by $H$. The function $R(H, w)$ takes a set of time steps $H$ and a robot behavior $w$ as input and returns a new behavior consisting only of the input and output values that occur at the time steps in $H$. In other words, it "projects" the original behavior onto the set of time steps in $H$.

 \begin{definition}[LTL Contract]
  A contract is a pair $\mathcal{C} = (\varphi_A, \varphi_G)$ of LTL specifications, where $\varphi_A$ denotes the behaviors assumed of the environment and $\varphi_G$ the behaviors the robot is allowed when the environment meets the assumptions. 
\end{definition}

 \begin{definition}[Goal]
    A goal is a pair $\mathcal{G}=(ctx, \mathcal{C})$ where $ctx$ is a Boolean formula and $\mathcal{C}$ is a contract. Let $G$ be the set of all goals in a mission.
    \end{definition}
    
    Intuitively, a goal $\mathcal{G}$ is an objective (formalized by the contract $\mathcal{C}_i$) that the robot must achieve during the mission under contexts where the condition $ctx$ holds. Let $x_t$ denote the context that is active at time $t$. We say that $ctx$ holds if $ctx \land x_t$ is satisfiable. At every time step, we say that a goal $\mathcal{G}=(ctx, \mathcal{C})$ is an \textbf{active goal} if its context $ctx$ is satisfiable with the currently active context $x_t$. With a slight abuse of notation, for the rest of the paper we refer to $ctx$ as the \textit{context} of the goal $\mathcal{G}$. A context is both a \textit{static} Boolean condition belonging to a goal (i.e. a \textit{goal context}), and a \textit{dynamic} Boolean condition evaluated over the natural numbers (i.e. a \textit{mission context}).
 
\begin{definition}[Mission]
    A contextual mission $\mathcal{M} = {(X, G)}$, or simply a mission, is a pair containing the set of all mission contexts and goals.
    \end{definition}
    
    Given a mission $\mathcal{M} = {(X, G)}$, we want to formulate for every context $x_i \in X$, the set of behaviours that the robot must satisfy when $x_i$ is active. These behaviours are produced by some combination of contracts belonging to goals which a are active when $x_i$ is active. We formulate such behaviours with \textit{mission scenarios}.
    
    \begin{definition}[Mission Scenario]
    A mission scenario is a pair $\mathcal{M}_i = {(x_i, \gamma_i)}$ where $x_i \in X$ and $\gamma_i$ is an LTL formula.
    \end{definition}
    A mission scenario indicates for every mutually exclusive context $x_i \in X$, the set of behaviours that must be satisfied by the robot. A mission scenario is \textit{active} when its context is active.
    
\begin{definition}[Active Signal]
    We define a Boolean condition $\mathcal{A} \in \mathcal{O}$ which we call \textit{active signal}. That is an output signal controlled by the robot, that at each time-step can be \textit{true} or \textit{false}.
\end{definition}

\noindent \textbf{Assumptions:} 
\begin{itemize}
    \item $\mathcal{A}$ becomes \textit{false} at every context-switch and stays \textit{false} for at most $t_{\texttt{trans}}$ time units, where $t_{\texttt{trans}} << t_{\texttt{context}}$.
\end{itemize}

\begin{definition}[Indexing Function]
    We define a function $I: X \times \mathcal{O} \rightarrow 2^{\mathbb{N}}$ that takes as input a context $x_i \in X$ and the active signal $\mathcal{A} \in \mathcal{O}$ and returns the set of natural numbers representing the time steps when $x_i$ and $\mathcal{A}$ are both \textit{true}.
\end{definition}

\vspace*{2mm}
\noindent

Given a mission $\mathcal{M} = \{X, G\}$, we can formulate two problems:

\vspace*{2mm}
\noindent{\textbf{Problem 1:}} For each context $x_i \in X$, produce a mission scenario $\mathcal{M}_i = (x_i, \gamma_i)$.

\vspace*{2mm}
\noindent{\textbf{Problem 2:}} For each mission scenario $\mathcal{M}_i = (x_i, \gamma_i)$, produce a robot behavior $w = w_0, w_1, w_2, \ldots$ such that
\begin{equation}
R(I(x_i, \mathcal{A}), w) \models \gamma_i
\end{equation}

In Problem 1, we aim to specify the set of behaviors that the robot must satisfy for each context. In Problem 2, we aim to generate a robot behavior that satisfies a given mission scenario by using the indexing function $I(x_i, \mathcal{A})$ to obtain the time steps when the context and active signal are both true.

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{figures/timeline-problem-fixed.pdf}
    \caption{Example of two contextual tasks active at different points in time.}
    \label{fig:timeline-problem}
\end{figure}  
  
\noindent Figure~\ref{fig:timeline-problem} illustrates an example of active contexts and mission scenarios between $t=0$ and $t=10$, where the overall robot behavior is denoted by $w$ and its projected robot behaviors $R(I(x_1, \mathcal{A}), w)$ and $R(I(x_3, \mathcal{A}), w)$ are shown. In order to satisfy the robotic mission, the following conditions must hold:
\begin{itemize}
\item $R(I(x_1, \mathcal{A}), w) = w_5, w_6 \dots \models \gamma_1$
\item $R(I(x_3, \mathcal{A}), w) = w_0, w_1, w_2, w_8, w_9, w_{10} \dots \models \gamma_3$
\end{itemize}

A contextual mission is satisfied if the robot behaves according to the allowed behaviors $\gamma_i$ of each mission scenario $\mathcal{M}_i = (x_i, \gamma_i)$ when $x_i$ is active. If a scenario becomes active after having been inactive, the robot resumes from where it left the last time the scenario was active. In Figure~\ref{fig:timeline-problem}, $\mathcal{M}_3=(x_3, \gamma_3)$ is the active scenario at step $t=0$. At step $t=3$, the context has changed from $x_3$ to $x_1$, resulting in a different scenario $\mathcal{M}_1$ becoming active. When the scenario $\mathcal{M}_3$ becomes active again at step $t=7$, the robot must \textit{resume} satisfying the behavior of $\gamma_3$ from when it left at time $t=2$, i.e., before the first context switch. We assume a maximum time frame $t{\texttt{trans}}$ after a context switch that allows the robot to adapt to the new scenario.

The upcoming sections describe how \NAME solves the previously presented problems. In Section~\ref{sec:cgg}, we explain how Problem 1 is addressed, while in Section~\ref{sec:orchestration}, we discuss how Problem 2 is tackled.



==> Tex/prome-definition-broken.tex <==

\section{Problem Definition}
\label{sec:problem}

Robotic missions specify what the robot should accomplish under different environmental conditions or \textit{contexts}. We model each robot objective in terms of \textit{goals} and formalize each goal in terms of \textit{contracts}. 

\pierl{Can we skip goals altogether and directly go to contracts? I think it will be simpler and cleaner.} \pierg{no, a goal includes a context, a contract does not}
We assume that time is discrete, and refer to a finite sequence of steps as a \textit{time interval} or \textit{frame}. We start by providing the definition of behavior and context. 

\begin{definition}[Behavior]
A behavior is a sequence of  assignments of values to all system (robot and environment) variables. 
\end{definition}

\begin{definition}[Context] A mission context $x$ is a sequence of Boolean assignments, i.e., $x: \mathbb{N} \rightarrow \{\textit{true}, \textit{false}\}$. We denote by $X$ the finite set of all the mission contexts  $X=\{x_0, x_1, \dots, x_n\}$.
\end{definition}
\pierl{This notation may create problem if you also need to describe the time behavior of a context. So, the context is just a behavior of some Boolean variable?}
    
    \noindent \textbf{Assumptions:}
    \begin{itemize}
    \item The contexts in $X$ are mutually exclusive. That is, for every $x_i, x_j \in X$, with $i \neq j$, if $x_i$ is \textit{true} at any time step, then $x_j$ must be \textit{false} at the same time step. \pierl{So, one context is always the complement of the other? Seems these definitions can be simplified?}
    \item Every context $x_i \in X$ is \textit{true} infinitely often, i.e., $\textsf{G}\textsf{F}x_i$ holds for all $x_i \in X$.
    \item Every context is \textit{true} for at least $t_{\texttt{context}}$ consecutive time steps. \pierl{more compact/meaningful subscript?}
    \end{itemize}
    
    A context represents a Boolean property of the robot's environment, such as whether it is raining or not, or whether it is day or night. 
    At any given step during the mission, at most one context is \textbf{active}, i.e., is \textit{true}. 
    A \textbf{context switch} is an uncontrolled event that can happen at any point during the execution of the mission. When a context switch occurs, the current active context becomes inactive, and a different context becomes active. Both events occur instantaneously at the same step. 
 
We model the robot as a set of behaviors over the variables in $\mathcal{I}$ and $\mathcal{O}$ representing the inputs and outputs of the robot, respectively.

\begin{definition}[Robot Behavior]
A robot behavior $w$ is a sequence of assignments to the variables in $\mathcal{I}$ and $\mathcal{O}$, that is, $w = (w_0^{\mathcal{I}}, w_0^{\mathcal{O}}),(w_1^{\mathcal{I}}, w_1^{\mathcal{O}}),(w_2^{\mathcal{I}}, w_2^{\mathcal{O}}), \ldots \in (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega$. We indicate with $w_t = (w_t^{\mathcal{I}}, w_t^{\mathcal{O}})$ the input and output values at time $t$. 
\end{definition}

\begin{definition}[Projected Robot Behavior]
    Given a function $R: 2^{\mathbb{N}} \times (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega \rightarrow (2^{\mathcal{I}} \times 2^{\mathcal{O}})^\omega$ that takes as inputs a tuple $H = (t_0, t_1, \ldots, t_h)$ of natural numbers, with $t_0 < t_1 < \ldots < t_h$ and a robot behavior $w$, the \textit{projected robot behavior} $R(H, w)$ is the trace $(w^{\mathcal{I}}_{t_0}, w^{\mathcal{O}}_{t_0}),(w^{\mathcal{I}}_{t_1}, w^{\mathcal{O}}_{t_1}), \ldots, (w^{\mathcal{I}}_{t_h}, w^{\mathcal{O}}_{t_h})$. 
\end{definition}
The projected robot behavior is obtained by restricting the robot behavior to the set of time steps specified by $H$. 

 \begin{definition}[LTL Contract]
  An LTL contract is a pair $\mathcal{C} = (\varphi_A, \varphi_G)$ of LTL formulas, where $\varphi_A$ denotes the behaviors assumed from the environment and $\varphi_G$ the behaviors the robot promises when the environment meets the assumptions. 
\end{definition}

\nir{Why isn't this just LTL?}

 \begin{definition}[Goal]
    A goal is a pair $\mathcal{G}=(x, \mathcal{C})$ where $x\in X$ is a context and $\mathcal{C}$ is a contract. 
    Let $G$ be the set $\{G_x\}_{x\in X}$ of contextual goals, which has a contract per context. \pierl{Confusing notation. What is an element of $G$. If it is a goal, should we use the notation for goals?}
    \end{definition}
    
    A goal $\mathcal{G}$ is an objective, formalized by the contract $\mathcal{C}_i$, that the robot must achieve during the mission under the context $x$. 
    Let $x_t$ denote the context that is active at time $t$. \pierl{This is very confusing. So far we have not used subscripts with this meaning for a context. A context is active infinitely often, then which index shall we choose?} We say that $x$ holds if $x= x_t$ \pierl{What does this mean?}. At time step $t$, we say that a goal $\mathcal{G}_x=(x, \mathcal{C})$ is \textbf{active} if its context $x$ is active at step $t$. 
    A context is both a \textit{static} value belonging to a goal (i.e., a \textit{goal context}), and a \textit{dynamic} condition that holds at a given time. \pierl{I don't understand what this sentence mean. A context is a behavior. How can it be a static value?}
 
\begin{definition}[Mission]
    A contextual mission $\mathcal{M} = {(X, G)}$, or simply a mission, is a pair containing a set of contexts and a set of goals.
\end{definition}
    
When a context changes, some time may be required in order to set up the conditions for the fulfillment of the goal of the new context. \pierl{This sentence is not clear. we said that context and goal switching is instantaneous and simultaneous.}  
We allow the robot to signal this using an \emph{active signal}.
\pierl{Don't understand what the robot needs to signal.}

\begin{definition}[Active Signal]
    We define a Boolean condition $\mathcal{A} \in \mathcal{O}$ which we call \textit{active signal}. That is an output signal controlled by the robot, that at each time-step can be \textit{true} or \textit{false}. \pierl{Revise definition. It is an output variable? Or a signal, hence a behavior?}
\end{definition}

The active signal is set to false whenever the context switches. \pierl{The word `active' is abused. Goal is active, context is active, active signal is active or inactive. Hard to follow, read, and understand.} We assume a maximal duration after which the active signal turns on again.

\noindent \textbf{Activity assumption:} 
    The active signal $\mathcal{A}$ becomes \textit{false} at every context switch and stays \textit{false} for at most $t_{\texttt{trans}}$ time units, where $t_{\texttt{trans}} << t_{\texttt{context}}$.

Using the active signal and the contexts, we can identify the time frame within \pierl{during?} which a goal associated with a certain context should be satisfied.

\begin{definition}[Indexing Function]
    We define a function $I: X \times \mathcal{O} \rightarrow 2^{\mathbb{N}}$ that takes as input a context $x_i \in X$ and the active signal $\mathcal{A} \in \mathcal{O}$ and returns the set of natural numbers representing the time steps when $x_i$ and $\mathcal{A}$ are both \textit{true}. \pierl{true or satisfied? Where does $w$ come from here? Also, why satisfaction. The right hand side should be a formula?} Namely, $I(x) = \{j 
     \in N ~|~ w_j \models x\wedge \mathcal{A}\}$.
\end{definition}

\vspace*{2mm}
\noindent

Given a mission $\mathcal{M} = (X, G)$, we can formulate the following problem:

\smallskip
\noindent{\textbf{Problem:}} 
For each goal $G_x=(x,\mathcal{C})$ produce a robot behavior $w = w_0, w_1, w_2, \ldots \in O^\omega$ such that
\begin{equation}
R(I(x_i, \mathcal{A}), w) \models \gamma_i 
\end{equation}
\pierl{Unclear.}

In Problem 1 \pierl{what is problem 1?}, we aim to specify the set of behaviors that the robot must satisfy for each context. In Problem 2 \pierl{???}, we aim to generate a robot behavior that satisfies a given mission scenario \pierl{what is a mission scenario?} by using the indexing function $I(x_i, \mathcal{A})$ to obtain the time steps when the context and active signal are both true. \pierl{why are we using an indexing function?}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{figures/timeline-problem.eps}
    \caption{Example of two contextual tasks active at different points in time.}
    \label{fig:timeline-problem}
\end{figure}
  
\noindent Figure~\ref{fig:timeline-problem} illustrates an example of active contexts and mission scenarios between $t=0$ and $t=10$, where the overall robot behavior is denoted by $w$ and its projected behaviors by $R(I(x_1, \mathcal{A}), w)$ and $R(I(x_2, \mathcal{A}), w)$. To satisfy the robotic mission, the following conditions must hold:
\begin{itemize}
\item $R(I(x_1, \mathcal{A}), w) = w_5, w_6 \dots \models \gamma_1$
\item $R(I(x_2, \mathcal{A}), w) = w_0, w_1, w_2, w_8, w_9, w_{10} \dots \models \gamma_2$
\end{itemize}

A contextual mission is satisfied if the robot behaves according to the prescribed behaviors $\gamma_i$ of each mission scenario $\mathcal{M}_i = (x_i, \gamma_i)$ when $x_i$ is active. \pierl{have we ever defined a scenario? what is $\gamma_i$? Is there a contract here?} If a scenario becomes active after having been inactive, the robot resumes from where it left the last time the scenario was active \pierl{what does it mean?}. In Figure~\ref{fig:timeline-problem}, $\mathcal{M}_2=(x_2, \gamma_2)$ is the active scenario at step $t=0$ \pierl{but you said that $x_2$ is active at time 2?}. At step $t=3$, the context has changed from $x_2$ to $x_1$, resulting in a different scenario $\mathcal{M}_1$ becoming active. When the scenario $\mathcal{M}_2$ becomes active again at step $t=7$, the robot must \textit{resume} satisfying the behavior of $\gamma_2$ from when it left at time $t=2$, i.e., before the first context switch. We assume a maximum time frame $t_{\texttt{trans}}$ after a context switch that allows the robot to adapt to the new scenario. \pierl{Very informal and the formalization of these behaviors of the robot is not clear in this section.}

The upcoming sections describe how \NAME solves the previously presented problems \pierl{???}. In Section~\ref{sec:cgg}, we explain how Problem 1 is addressed, while in Section~\ref{sec:orchestration}, we discuss how Problem 2 is tackled.
\nir{\NAME is not properly introduced.}



==> Tex/related_orig.tex <==

\section{Related Work}\label{sec:related}

Despite the valuable contributions to the state-of-the-art in the field, to the best of our knowledge,  dealing with the variability of the environment and addressing context switching are still open problems. In this section, we present works that are related to mission specifications (Section~\ref{sec:missionSpecification}) and reactive synthesis applied to robotics (Section~\ref{sec:reactiveSynthesis}). We also have a brief discussion about the concept of context (Section~\ref{sec:bncontext}).

\subsection{Mission Specification}\label{sec:missionSpecification}

A robotic mission is usually defined as a set of tasks or goals that a robot must accomplish.
Different approaches have been proposed for specifying missions, including the use of logics~\cite{menghi2018multi,ulusoy2011optimal,fainekos2009temporal,guo2013revising,wolff2013automaton,kress2011robot,doi:10.1177/0278364914546174}, state charts~\cite{bohren2010smach,thomas2013new,klotzbucher2012coordinating}, and Petri Nets~\cite{wang1991petri,ziparo2008petri}. However, the exposure to formal methods, often required to use these formalisms can be a hindrance to their wider adoption.
Various domain-specific languages (DSLs) have been proposed to make mission specification more accessible~\cite{GLRSWWCA12,campusano.ea:2017:live,DBLP:journals/corr/SchwartzNAM14,Ruscio2016,Bozhinoski2015,Ciccozzi4496,Doherty2012}. These DSLs provide a high-level and easy-to-use interface for mission specification.

A recent survey by Dreagule et al.~\cite{dragule2021b} on domain-specific languages for robot mission specifications, classifies them into internal and external DSLs, and provides an overview of their tooling support. Moreover, robotic patterns have been proposed as a solution to recurrent mission specification problems~\cite{SpecificationPatternsTSE}. The PsALM tool~\cite{PSALM} enables the specification of robotic missions using mission specification patterns, which capture robot movements and actions performed as a robot moves in the environment. \NAME supports 22 patterns~\cite{SpecificationPatternsTSE} that cover various mission requirements, organized into three groups: core movement patterns, triggers, and avoidance patterns. For example, the \textit{Strict Ordered Patrolling} pattern\footnote{\url{http://roboticpatterns.com/pattern/strictorderedpatrolling/}} can be used to specify the requirement that a robot must patrol a set of locations in a specific strict order, with each location represented by an atomic proposition. Let $l_1, l_2$, and $l_3$ be the atomic propositions of type \textit{location} that the robot must visit in the given order. 
The mission requirement can then be reformulated as `Given locations $l_1, l_2$, and $l_3$, the robot should visit all the locations indefinitely and following a strict order,' leading to the following LTL formulation:
\begin{align}
& \mathbf{G}(\mathbf{F}(l_1 \land \mathbf{F}(l_2 \land \mathbf{F}(l_3)))) \land (\overline{l_2} ~\mathbf{U}~l_1) \land (\overline{l_3} ~\mathbf{U}~l_2) \nonumber\\
\land~ & \mathbf{G}(l_2 \rightarrow \mathbf{X}(\overline{l_2} ~\mathbf{U}~ l_1)) \land \mathbf{G}(l_3 \rightarrow \mathbf{X}(\overline{l_3} ~\mathbf{U}~ l_2)) \\
\land ~ & \mathbf{G}(l_1 \rightarrow \mathbf{X}(\overline{l_1} ~\mathbf{U}~ l_3)) \nonumber\\
\land~ & \mathbf{G}(l_1 \rightarrow \mathbf{X}(\overline{l_1} ~\mathbf{U}~ l_2)) \land \mathbf{G}(l_2 \rightarrow \mathbf{X}(\overline{l_2} ~\mathbf{U}~ l_3)). \nonumber
\end{align}
As shown in this example, a robotic pattern can significantly facilitate the error-prone and challenging task of mission specification.  

Despite all the efforts described above, formalizing mission requirements in specifications is still considered to be a challenge. 
\NAME utilizes a catalog of patterns~\cite{patterns, dywerpatterslink} as a tool to express formally, but still intuitively, what the robot should do.

\subsection{Context}\label{sec:bncontext}

The concept of context has been widely discussed in the literature, with various definitions proposed. In the field of ubiquitous computing, context can include information such as location, time of day, nearby objects and people, and temperature~\cite{Krumm2010}. Dey and Abowd~\cite{dey2001understanding} define context more broadly as any information that can be used to characterize the situation of an entity, including the user and application themselves. In robotics, Bloisi et al.~\cite{Bloisi2016} define mission-related contexts as choices that enable robots to adapt their behavior to different situations.

One of the most challenging aspects of specifying robotic missions is capturing the exceptional behaviors that robots must exhibit to cope with the variability of conditions in real-world environments~\cite{ESECFSE2020}. To address this challenge, \NAME formalizes context as a property associated with a goal and expressed by a logic formula, building on existing characterizations of context. This approach allows for the specification of exceptional behaviors that a robot must exhibit in response to changing environmental conditions.

\subsection{Reactive Synthesis}\label{sec:reactiveSynthesis}

Reactive synthesis has been applied in robotics for synthesizing controllers. A compositional approach to reactive synthesis was introduced~\cite{Moshe2019} for finite-horizon tasks represented using formulas of linear temporal logic on finite traces (LTLf). The work in~\cite{Salar2018} presents algorithms to synthesize controllers for a swarm robotic system. The work in~\cite{MaozRose} identifies some software engineering challenges in applying reactive synthesis to robotics, including the synthesis algorithms themselves, adequate development processes and tools, declarative specification writing, and abstraction of data and time.

To address the challenge of dealing with the variability of conditions in real-world environments where robots operate, highlighted in Section~\ref{sec:missionSpecification}, one approach is to decompose the mission specification into sub-mission specifications, each activated in particular contexts and conditions. The work in~\cite{nahabedian_2020} proposes the automatic computation of a controller to handle the transition from one specification to another. However, the synthesis of controllers is done at runtime, which may cause problems if there is an immediate need to switch from one controller to another. The work in~\cite{ippolito2014_hope} proposes a hierarchy of discrete event controllers that support graceful degradation when the assumptions of a higher-level controller are broken and progressive enhancement when those assumptions are satisfied or restored. This approach allows for instantaneous switching and offers guarantees regarding behaviors across controller switches, but it requires predefined layers organized into a strict logical implication order.

\NAME is an end-to-end solution that addresses the problem of specifying and realizing contextual mission specifications. It simplifies mission specification by decomposing the mission into a set of context-dependent sub-missions. Once the mission is specified in a set of context-dependent sub-missions, \NAME automatically synthesizes (i) a controller for each sub-mission that satisfies the contextual mission and (ii) an orchestrator of the different controllers to support context switching during the mission to satisfy the overall contextual mission. The synthesis of the controllers uses reactive synthesis techniques, and unlike the work in~\cite{nahabedian_2020}, the same contexts can switch back and forth indefinitely while the controllers are being manipulated by the orchestrator.


